Chaos and order in event-triggered control

Event-triggered control (ETC) is claimed to provide enormous reductions in sampling frequency when compared to periodic sampling, but little is formally known about its generated traffic. This work shows that ETC can exhibit very complex, even chaotic traffic, especially when the triggering condition is aggressive in reducing communications. First, we characterize limit traffic patterns by observing invariant lines and planes through the origin, as well as their attractivity. Then, we present abstraction-based methods to compute limit metrics, such as limit average and limit inferior inter-sample time (IST) of periodic ETC (PETC), with considerations to the robustness of such metrics, as well as measuring the emergence of chaos. The methodology and tools allow us to find ETC examples that provably outperform periodic sampling in terms of average IST. In particular for PETC, we prove that this requires aperiodic or chaotic traffic.

==> figures/ex1_case2_PETC_data.tex <==
\addplot [semithick, blue]
table {%
-1.5707963267949 1.44180177950074
-1.5697963267949 1.44336691628846
-1.5687963267949 1.4449315477312
-1.5677963267949 1.44649566978538
-1.5667963267949 1.44805927778306
-1.5657963267949 1.44962236764264
-1.5647963267949 1.4511849351214
-1.5637963267949 1.45274697596622
-1.5627963267949 1.45430848594694
-1.5617963267949 1.45586946084455
-1.5607963267949 1.45742989645121
-1.5597963267949 1.45898978857036
-1.5587963267949 1.46054913301676
-1.5577963267949 1.46210792561658
-1.5567963267949 1.46366616220745
-1.5557963267949 1.46522383863856
-1.5547963267949 1.46678095077072
-1.5537963267949 1.46833749447641
-1.5527963267949 1.4698934656399
-1.5517963267949 1.47144886015725
-1.5507963267949 1.47300367393644
-1.5497963267949 1.47455790289742
-1.5487963267949 1.47611154297214
-1.5477963267949 1.47766459010179
-1.5467963267949 1.47921704024555
-1.5457963267949 1.48076888937214
-1.5447963267949 1.48232013346229
-1.5437963267949 1.4838707685091
-1.5427963267949 1.4854207905181
-1.5417963267949 1.48697019550732
-1.5407963267949 1.48851897950733
-1.5397963267949 1.49006713856134
-1.5387963267949 1.49161466872521
-1.5377963267949 1.49316156606758
-1.5367963267949 1.49470782666986
-1.5357963267949 1.49625344662634
-1.5347963267949 1.49779842204423
-1.5337963267949 1.49934274904372
-1.5327963267949 1.50088642375806
-1.5317963267949 1.50242944233362
-1.5307963267949 1.50397180092993
-1.5297963267949 1.50551349571981
-1.5287963267949 1.50705452288946
-1.5277963267949 1.50859487863823
-1.5267963267949 1.51013455917695
-1.5257963267949 1.511673560733
-1.5247963267949 1.51321187954562
-1.5237963267949 1.51474951186771
-1.5227963267949 1.5162864539658
-1.5217963267949 1.51782270212009
-1.5207963267949 1.5193582526245
-1.5197963267949 1.52089310178668
-1.5187963267949 1.52242724592807
-1.5177963267949 1.52396068138397
-1.5167963267949 1.52549340450353
-1.5157963267949 1.52702541164987
-1.5147963267949 1.52855669920008
-1.5137963267949 1.53008726354526
-1.5127963267949 1.53161710109059
-1.5117963267949 1.53314620825538
-1.5107963267949 1.53467458147308
-1.5097963267949 1.53620221719135
-1.5087963267949 1.53772911187211
-1.5077963267949 1.53925526199155
-1.5067963267949 1.54078066404022
-1.5057963267949 1.54230531452301
-1.5047963267949 1.54382920995925
-1.5037963267949 1.54535234688273
-1.5027963267949 1.5468747218417
-1.5017963267949 1.54839633139899
-1.5007963267949 1.54991717213196
-1.4997963267949 1.55143724063262
-1.4987963267949 1.55295653350752
-1.4977963267949 1.55447504737108
-1.4967963267949 1.55599277886876
-1.4957963267949 1.55750972465116
-1.4947963267949 1.55902588138373
-1.49379632679491 1.5605412457468
-1.49279632679491 1.56205581443563
-1.49179632679491 1.56356958416041
-1.49079632679491 1.56508255164629
-1.48979632679491 1.56659471363345
-1.48879632679491 1.56810606687705
-1.48779632679491 1.56961660813036
};
\addplot [semithick, blue]
table {%
-1.48679632679491 -1.57046631939696
-1.48579632679491 -1.56895741172521
-1.48479632679491 -1.56744932562898
-1.48379632679491 -1.5659420642779
-1.48279632679491 -1.56443563082645
-1.48179632679491 -1.56293002841391
-1.48079632679491 -1.56142526016434
-1.47979632679491 -1.55992132918654
-1.47879632679491 -1.55841823857401
-1.47779632679491 -1.55691599140494
-1.47679632679491 -1.55541459074207
-1.47579632679491 -1.55391403932277
-1.47479632679491 -1.55241434079469
-1.47379632679491 -1.55091549786984
-1.47279632679491 -1.54941751354972
-1.47179632679491 -1.54792039082041
-1.47079632679491 -1.54642413265256
-1.46979632679491 -1.54492874200136
-1.46879632679491 -1.54343422180653
-1.46779632679491 -1.54194057499227
-1.46679632679491 -1.54044780446729
-1.46579632679491 -1.53895591312477
-1.46479632679491 -1.53746490384233
-1.46379632679491 -1.53597477948204
-1.46279632679491 -1.53448554289038
-1.46179632679491 -1.53299719689824
-1.46079632679491 -1.5315097443209
-1.45979632679491 -1.53002318795804
-1.45879632679491 -1.52853753059368
-1.45779632679491 -1.52705277499621
-1.45679632679491 -1.52556892391835
-1.45579632679491 -1.52408598009715
-1.45479632679491 -1.522603946254
-1.45379632679491 -1.52112282509457
-1.45279632679491 -1.51964261930886
-1.45179632679491 -1.51816333157113
-1.45079632679491 -1.51668496453995
-1.44979632679491 -1.51520752085814
-1.44879632679491 -1.51373100315281
-1.44779632679491 -1.51225541403531
-1.44679632679491 -1.51078075610125
-1.44579632679491 -1.50930703193049
-1.44479632679491 -1.50783424408713
-1.44379632679491 -1.50636239511951
-1.44279632679491 -1.50489148756022
-1.44179632679491 -1.50342152392604
-1.44079632679491 -1.50195250671801
-1.43979632679491 -1.50048443842138
-1.43879632679491 -1.49901732150564
-1.43779632679491 -1.49755115842448
-1.43679632679491 -1.49608595161582
-1.43579632679491 -1.49462170350181
-1.43479632679491 -1.49315841648879
-1.43379632679491 -1.49169609296735
-1.43279632679491 -1.4902347353123
-1.43179632679491 -1.48877434588265
-1.43079632679491 -1.48731492702166
-1.42979632679491 -1.48585648105681
-1.42879632679491 -1.4843990102998
-1.42779632679491 -1.48294251704659
-1.42679632679491 -1.48148700357736
-1.42579632679491 -1.48003247215654
-1.42479632679491 -1.47857892503281
-1.42379632679491 -1.47712636443911
-1.42279632679491 -1.47567479259263
-1.42179632679491 -1.47422421169483
-1.42079632679491 -1.47277462393146
-1.41979632679491 -1.47132603147254
-1.41879632679491 -1.46987843647238
-1.41779632679491 -1.4684318410696
-1.41679632679491 -1.46698624738711
-1.41579632679491 -1.46554165753216
-1.41479632679491 -1.46409807359632
-1.41379632679491 -1.4626554976555
-1.41279632679491 -1.46121393176994
-1.41179632679491 -1.45977337798428
-1.41079632679491 -1.45833383832751
-1.40979632679491 -1.456895314813
-1.40879632679491 -1.45545780943853
-1.40779632679491 -1.45402132418628
-1.40679632679491 -1.45258586102288
-1.40579632679491 -1.45115142189936
-1.40479632679491 -1.44971800875124
-1.40379632679491 -1.4482856234985
-1.40279632679492 -1.44685426804559
-1.40179632679492 -1.44542394428147
-1.40079632679492 -1.44399465407962
-1.39979632679492 -1.44256639929805
-1.39879632679492 -1.44113918177932
-1.39779632679492 -1.43971300335056
-1.39679632679492 -1.43828786582347
-1.39579632679492 -1.43686377099438
-1.39479632679492 -1.43544072064423
-1.39379632679492 -1.4340187165386
-1.39279632679492 -1.43259776042774
-1.39179632679492 -1.43117785404658
-1.39079632679492 -1.42975899911474
-1.38979632679492 -1.42834119733657
-1.38879632679492 -1.42692445040118
-1.38779632679492 -1.42550875998242
-1.38679632679492 -1.42409412773896
-1.38579632679492 -1.42268055531423
-1.38479632679492 -1.42126804433655
-1.38379632679492 -1.41985659641906
-1.38279632679492 -1.41844621315979
-1.38179632679492 -1.41703689614166
-1.38079632679492 -1.41562864693255
-1.37979632679492 -1.41422146708525
-1.37879632679492 -1.41281535813757
-1.37779632679492 -1.41141032161228
-1.37679632679492 -1.41000635901709
-1.37579632679492 -1.40860347184494
-1.37479632679492 -1.40720166157381
-1.37379632679492 -1.40580092966679
-1.37279632679492 -1.40440127757205
-1.37179632679492 -1.40300270672295
-1.37079632679492 -1.40160521853803
-1.36979632679492 -1.40020881442105
-1.36879632679492 -1.39881349576102
-1.36779632679492 -1.3974192639322
-1.36679632679492 -1.39602612029418
-1.36579632679492 -1.39463406619187
-1.36479632679492 -1.39324310295554
-1.36379632679492 -1.39185323190086
-1.36279632679492 -1.3904644543289
-1.36179632679492 -1.38907677152622
-1.36079632679492 -1.38769018476482
-1.35979632679492 -1.38630469530224
-1.35879632679492 -1.38492030438157
-1.35779632679492 -1.38353701323145
-1.35679632679492 -1.38215482306615
-1.35579632679492 -1.38077373508559
-1.35479632679492 -1.37939375047533
-1.35379632679492 -1.37801487040668
-1.35279632679492 -1.37663709603665
-1.35179632679492 -1.37526042850804
-1.35079632679492 -1.37388486894947
-1.34979632679492 -1.37251041847538
-1.34879632679492 -1.3711370781861
-1.34779632679492 -1.36976484916785
-1.34679632679492 -1.36839373249281
-1.34579632679492 -1.36702372916834
-1.34479632679492 -1.36565484034404
-1.34379632679492 -1.3642870669955
-1.34279632679492 -1.36292041013901
-1.34179632679492 -1.36155487077702
-1.34079632679492 -1.36019044989809
-1.33979632679492 -1.35882714847702
-1.33879632679492 -1.35746496747479
-1.33779632679492 -1.35610390783869
-1.33679632679492 -1.3547439705023
-1.33579632679492 -1.35338515638553
-1.33479632679492 -1.35202746639469
-1.33379632679492 -1.35067090142249
-1.33279632679492 -1.3493154623481
-1.33179632679492 -1.34796115003719
-1.33079632679492 -1.34660796534195
-1.32979632679492 -1.34525590910115
-1.32879632679492 -1.34390498214015
-1.32779632679492 -1.34255518527099
-1.32679632679492 -1.34120651929238
-1.32579632679492 -1.33985898498973
-1.32479632679492 -1.33851258313527
-1.32379632679492 -1.33716731448798
-1.32279632679492 -1.33582317979373
-1.32179632679492 -1.33448017978525
-1.32079632679492 -1.3331383151822
-1.31979632679492 -1.33179758669121
-1.31879632679492 -1.33045799500592
-1.31779632679492 -1.329119540807
-1.31679632679492 -1.32778222476224
-1.31579632679492 -1.32644604752654
-1.31479632679492 -1.32511100974195
-1.31379632679492 -1.32377711203778
-1.31279632679492 -1.32244435503055
-1.31179632679493 -1.3211127393241
-1.31079632679493 -1.31978226550961
-1.30979632679493 -1.31845293416562
-1.30879632679493 -1.31712474585811
-1.30779632679493 -1.31579770114051
-1.30679632679493 -1.31447180055377
-1.30579632679493 -1.31314704462638
-1.30479632679493 -1.31182343387442
-1.30379632679493 -1.31050096880162
-1.30279632679493 -1.30917964989937
-1.30179632679493 -1.30785947764678
-1.30079632679493 -1.30654045251074
-1.29979632679493 -1.30522257494593
-1.29879632679493 -1.3039058453949
-1.29779632679493 -1.30259026428808
-1.29679632679493 -1.30127583204384
-1.29579632679493 -1.29996254906853
-1.29479632679493 -1.29865041575653
-1.29379632679493 -1.29733943249028
-1.29279632679493 -1.29602959964035
-1.29179632679493 -1.29472091756546
-1.29079632679493 -1.29341338661253
-1.28979632679493 -1.29210700711673
-1.28879632679493 -1.29080177940151
-1.28779632679493 -1.28949770377866
-1.28679632679493 -1.28819478054837
-1.28579632679493 -1.28689300999923
-1.28479632679493 -1.28559239240831
-1.28379632679493 -1.28429292804119
-1.28279632679493 -1.28299461715201
-1.28179632679493 -1.28169745998352
-1.28079632679493 -1.28040145676711
-1.27979632679493 -1.27910660772288
-1.27879632679493 -1.27781291305965
-1.27779632679493 -1.27652037297504
-1.27679632679493 -1.2752289876555
-1.27579632679493 -1.27393875727634
-1.27479632679493 -1.2726496820018
-1.27379632679493 -1.2713617619851
-1.27279632679493 -1.27007499736846
-1.27179632679493 -1.26878938828315
-1.27079632679493 -1.26750493484957
-1.26979632679493 -1.26622163717723
-1.26879632679493 -1.26493949536487
-1.26779632679493 -1.26365850950045
-1.26679632679493 -1.26237867966123
-1.26579632679493 -1.26110000591379
-1.26479632679493 -1.2598224883141
-1.26379632679493 -1.25854612690755
-1.26279632679493 -1.25727092172899
-1.26179632679493 -1.2559968728028
-1.26079632679493 -1.25472398014292
-1.25979632679493 -1.25345224375288
-1.25879632679493 -1.2521816636259
-1.25779632679493 -1.25091223974486
-1.25679632679493 -1.24964397208242
-1.25579632679493 -1.248376860601
-1.25479632679493 -1.24711090525289
-1.25379632679493 -1.24584610598024
-1.25279632679493 -1.24458246271515
-1.25179632679493 -1.24331997537968
-1.25079632679493 -1.24205864388593
-1.24979632679493 -1.24079846813604
-1.24879632679493 -1.2395394480223
-1.24779632679493 -1.23828158342713
-1.24679632679493 -1.23702487422318
-1.24579632679493 -1.23576932027336
-1.24479632679493 -1.23451492143084
-1.24379632679493 -1.23326167753917
-1.24279632679493 -1.23200958843228
-1.24179632679493 -1.23075865393455
-1.24079632679493 -1.22950887386082
-1.23979632679493 -1.22826024801648
-1.23879632679493 -1.22701277619749
-1.23779632679493 -1.22576645819043
-1.23679632679493 -1.22452129377254
-1.23579632679493 -1.22327728271179
-1.23479632679493 -1.22203442476691
-1.23379632679493 -1.22079271968741
-1.23279632679493 -1.21955216721368
-1.23179632679493 -1.21831276707699
-1.23079632679493 -1.21707451899957
-1.22979632679493 -1.21583742269461
-1.22879632679493 -1.21460147786638
-1.22779632679493 -1.21336668421018
-1.22679632679493 -1.21213304141246
-1.22579632679493 -1.21090054915085
-1.22479632679493 -1.20966920709419
-1.22379632679493 -1.20843901490258
-1.22279632679493 -1.20720997222742
-1.22179632679493 -1.20598207871148
-1.22079632679494 -1.20475533398892
-1.21979632679494 -1.20352973768535
-1.21879632679494 -1.20230528941787
-1.21779632679494 -1.2010819887951
-1.21679632679494 -1.19985983541725
-1.21579632679494 -1.19863882887618
-1.21479632679494 -1.19741896875537
-1.21379632679494 -1.19620025463006
-1.21279632679494 -1.19498268606723
-1.21179632679494 -1.19376626262567
-1.21079632679494 -1.19255098385603
-1.20979632679494 -1.19133684930082
-1.20879632679494 -1.19012385849454
-1.20779632679494 -1.18891201096363
-1.20679632679494 -1.18770130622659
-1.20579632679494 -1.18649174379398
-1.20479632679494 -1.18528332316849
-1.20379632679494 -1.18407604384494
-1.20279632679494 -1.1828699053104
-1.20179632679494 -1.18166490704416
-1.20079632679494 -1.18046104851782
-1.19979632679494 -1.17925832919531
-1.19879632679494 -1.17805674853296
-1.19779632679494 -1.17685630597951
-1.19679632679494 -1.17565700097618
-1.19579632679494 -1.1744588329567
-1.19479632679494 -1.17326180134736
-1.19379632679494 -1.17206590556705
-1.19279632679494 -1.17087114502732
-1.19179632679494 -1.16967751913239
-1.19079632679494 -1.16848502727922
-1.18979632679494 -1.16729366885755
-1.18879632679494 -1.16610344324995
-1.18779632679494 -1.16491434983182
-1.18679632679494 -1.16372638797149
-1.18579632679494 -1.16253955703023
-1.18479632679494 -1.16135385636231
-1.18379632679494 -1.16016928531503
-1.18279632679494 -1.15898584322875
-1.18179632679494 -1.15780352943697
-1.18079632679494 -1.15662234326635
-1.17979632679494 -1.15544228403674
-1.17879632679494 -1.15426335106125
-1.17779632679494 -1.15308554364628
-1.17679632679494 -1.15190886109153
-1.17579632679494 -1.15073330269012
-1.17479632679494 -1.14955886772855
-1.17379632679494 -1.14838555548678
-1.17279632679494 -1.14721336523828
-1.17179632679494 -1.14604229625006
-1.17079632679494 -1.14487234778269
-1.16979632679494 -1.14370351909039
-1.16879632679494 -1.14253580942101
-1.16779632679494 -1.14136921801615
-1.16679632679494 -1.14020374411111
-1.16579632679494 -1.139039386935
-1.16479632679494 -1.13787614571076
-1.16379632679494 -1.13671401965518
-1.16279632679494 -1.13555300797898
-1.16179632679494 -1.13439310988682
-1.16079632679494 -1.13323432457735
-1.15979632679494 -1.13207665124324
-1.15879632679494 -1.13092008907125
-1.15779632679494 -1.12976463724223
-1.15679632679494 -1.1286102949312
-1.15579632679494 -1.12745706130734
-1.15479632679494 -1.1263049355341
-1.15379632679494 -1.12515391676917
-1.15279632679494 -1.12400400416456
-1.15179632679494 -1.12285519686662
-1.15079632679494 -1.12170749401609
-1.14979632679494 -1.12056089474815
-1.14879632679494 -1.11941539819242
-1.14779632679494 -1.11827100347306
-1.14679632679494 -1.11712770970873
-1.14579632679494 -1.1159855160127
-1.14479632679494 -1.11484442149286
-1.14379632679494 -1.11370442525174
-1.14279632679494 -1.1125655263866
-1.14179632679494 -1.1114277239894
-1.14079632679494 -1.1102910171469
-1.13979632679494 -1.10915540494065
-1.13879632679494 -1.10802088644706
};
\addplot [semithick, blue]
table {%
-1.13779632679494 -1.04236076926161
-1.13679632679494 -1.04119201051185
-1.13579632679494 -1.04002559212877
-1.13479632679494 -1.03886150792829
-1.13379632679494 -1.03769975173508
-1.13279632679494 -1.03654031738261
-1.13179632679494 -1.0353831987133
-1.13079632679495 -1.03422838957859
-1.12979632679495 -1.03307588383898
-1.12879632679495 -1.03192567536419
-1.12779632679495 -1.0307777580332
-1.12679632679495 -1.02963212573435
-1.12579632679495 -1.02848877236542
-1.12479632679495 -1.02734769183368
-1.12379632679495 -1.02620887805603
-1.12279632679495 -1.02507232495903
-1.12179632679495 -1.023938026479
-1.12079632679495 -1.02280597656207
-1.11979632679495 -1.0216761691643
-1.11879632679495 -1.02054859825169
-1.11779632679495 -1.01942325780031
-1.11679632679495 -1.01830014179634
-1.11579632679495 -1.01717924423613
-1.11479632679495 -1.0160605591263
-1.11379632679495 -1.01494408048379
-1.11279632679495 -1.01382980233591
-1.11179632679495 -1.01271771872042
-1.11079632679495 -1.0116078236856
-1.10979632679495 -1.01050011129028
-1.10879632679495 -1.00939457560396
-1.10779632679495 -1.00829121070678
-1.10679632679495 -1.00719001068968
-1.10579632679495 -1.00609096965437
-1.10479632679495 -1.00499408171344
-1.10379632679495 -1.00389934099038
-1.10279632679495 -1.00280674161968
-1.10179632679495 -1.00171627774682
-1.10079632679495 -1.00062794352837
-1.09979632679495 -0.999541733132015
-1.09879632679495 -0.998457640736622
-1.09779632679495 -0.997375660532274
-1.09679632679495 -0.996295786720323
-1.09579632679495 -0.995218013513434
-1.09479632679495 -0.994142335135633
-1.09379632679495 -0.993068745822347
-1.09279632679495 -0.991997239820451
-1.09179632679495 -0.990927811388306
-1.09079632679495 -0.989860454795805
-1.08979632679495 -0.988795164324407
-1.08879632679495 -0.987731934267182
-1.08779632679495 -0.986670758928844
-1.08679632679495 -0.985611632625794
-1.08579632679495 -0.98455454968615
-1.08479632679495 -0.983499504449787
-1.08379632679495 -0.98244649126837
-1.08279632679495 -0.981395504505387
-1.08179632679495 -0.980346538536183
-1.08079632679495 -0.97929958774799
-1.07979632679495 -0.978254646539961
-1.07879632679495 -0.977211709323196
-1.07779632679495 -0.976170770520775
-1.07679632679495 -0.975131824567786
-1.07579632679495 -0.974094865911349
-1.07479632679495 -0.973059889010646
-1.07379632679495 -0.972026888336949
-1.07279632679495 -0.97099585837364
-1.07179632679495 -0.969966793616239
-1.07079632679495 -0.968939688572426
-1.06979632679495 -0.967914537762066
-1.06879632679495 -0.966891335717228
-1.06779632679495 -0.965870076982209
-1.06679632679495 -0.964850756113554
-1.06579632679495 -0.963833367680075
-1.06479632679495 -0.96281790626287
-1.06379632679495 -0.961804366455344
-1.06279632679495 -0.960792742863222
-1.06179632679495 -0.959783030104572
-1.06079632679495 -0.958775222809815
-1.05979632679495 -0.957769315621747
-1.05879632679495 -0.956765303195549
-1.05779632679495 -0.955763180198802
-1.05679632679495 -0.954762941311505
-1.05579632679495 -0.953764581226083
-1.05479632679495 -0.9527680946474
-1.05379632679495 -0.951773476292774
-1.05279632679495 -0.950780720891984
-1.05179632679495 -0.949789823187285
-1.05079632679495 -0.948800777933412
-1.04979632679495 -0.947813579897596
-1.04879632679495 -0.946828223859566
-1.04779632679495 -0.945844704611562
-1.04679632679495 -0.944863016958341
-1.04579632679495 -0.943883155717184
-1.04479632679495 -0.942905115717899
-1.04379632679495 -0.941928891802835
-1.04279632679495 -0.940954478826878
-1.04179632679495 -0.93998187165746
-1.04079632679495 -0.939011065174566
-1.03979632679496 -0.938042054270732
-1.03879632679496 -0.937074833851049
-1.03779632679496 -0.936109398833172
-1.03679632679496 -0.935145744147313
-1.03579632679496 -0.93418386473625
-1.03479632679496 -0.933223755555321
-1.03379632679496 -0.932265411572434
-1.03279632679496 -0.931308827768056
-1.03179632679496 -0.930353999135221
-1.03079632679496 -0.929400920679526
-1.02979632679496 -0.928449587419131
-1.02879632679496 -0.927499994384754
-1.02779632679496 -0.926552136619671
-1.02679632679496 -0.925606009179716
-1.02579632679496 -0.924661607133273
-1.02479632679496 -0.923718925561274
-1.02379632679496 -0.922777959557197
-1.02279632679496 -0.921838704227059
-1.02179632679496 -0.920901154689414
-1.02079632679496 -0.919965306075343
-1.01979632679496 -0.919031153528454
-1.01879632679496 -0.918098692204873
-1.01779632679496 -0.917167917273237
-1.01679632679496 -0.916238823914687
-1.01579632679496 -0.915311407322865
-1.01479632679496 -0.914385662703899
-1.01379632679496 -0.913461585276404
-1.01279632679496 -0.912539170271464
-1.01179632679496 -0.911618412932631
-1.01079632679496 -0.910699308515912
-1.00979632679496 -0.909781852289761
-1.00879632679496 -0.908866039535069
-1.00779632679496 -0.907951865545154
-1.00679632679496 -0.907039325625748
-1.00579632679496 -0.906128415094992
-1.00479632679496 -0.905219129283419
-1.00379632679496 -0.904311463533946
-1.00279632679496 -0.90340541320186
-1.00179632679496 -0.902500973654809
-1.00079632679496 -0.901598140272785
-0.999796326794959 -0.900696908448118
-0.99879632679496 -0.899797273585455
-0.99779632679496 -0.898899231101754
-0.99679632679496 -0.898002776426266
-0.99579632679496 -0.897107905000522
-0.99479632679496 -0.896214612278319
-0.99379632679496 -0.89532289372571
-0.99279632679496 -0.894432744820978
-0.99179632679496 -0.893544161054636
-0.99079632679496 -0.892657137929398
-0.989796326794961 -0.891771670960173
-0.988796326794961 -0.890887755674045
-0.987796326794961 -0.890005387610258
-0.986796326794961 -0.8891245623202
-0.985796326794961 -0.888245275367385
-0.984796326794961 -0.88736752232744
-0.983796326794961 -0.886491298788083
-0.982796326794961 -0.88561660034911
-0.981796326794961 -0.884743422622377
-0.980796326794962 -0.883871761231778
-0.979796326794962 -0.883001611813234
-0.978796326794962 -0.882132970014669
-0.977796326794962 -0.881265831495998
-0.976796326794962 -0.8804001919291
-0.975796326794962 -0.879536046997809
-0.974796326794962 -0.878673392397885
-0.973796326794962 -0.877812223837005
-0.972796326794962 -0.876952537034735
-0.971796326794963 -0.876094327722517
-0.970796326794963 -0.875237591643647
-0.969796326794963 -0.874382324553251
-0.968796326794963 -0.873528522218274
-0.967796326794963 -0.872676180417451
-0.966796326794963 -0.871825294941293
-0.965796326794963 -0.87097586159206
-0.964796326794963 -0.870127876183748
-0.963796326794963 -0.869281334542062
-0.962796326794964 -0.868436232504398
-0.961796326794964 -0.867592565919819
-0.960796326794964 -0.866750330649038
-0.959796326794964 -0.865909522564392
-0.958796326794964 -0.865070137549824
-0.957796326794964 -0.864232171500859
-0.956796326794964 -0.863395620324581
-0.955796326794964 -0.862560479939615
-0.954796326794964 -0.861726746276101
-0.953796326794965 -0.860894415275671
-0.952796326794965 -0.860063482891433
-0.951796326794965 -0.859233945087938
-0.950796326794965 -0.858405797841169
-0.949796326794965 -0.857579037138506
-0.948796326794965 -0.856753658978714
-0.947796326794965 -0.855929659371912
-0.946796326794965 -0.855107034339553
-0.945796326794965 -0.854285779914403
-0.944796326794966 -0.853465892140511
-0.943796326794966 -0.852647367073192
-0.942796326794966 -0.851830200778998
-0.941796326794966 -0.8510143893357
-0.940796326794966 -0.850199928832259
-0.939796326794966 -0.849386815368804
-0.938796326794966 -0.848575045056607
-0.937796326794966 -0.847764614018062
-0.936796326794966 -0.846955518386656
-0.935796326794966 -0.846147754306948
-0.934796326794967 -0.845341317934543
-0.933796326794967 -0.844536205436068
-0.932796326794967 -0.843732412989148
-0.931796326794967 -0.84292993678238
-0.930796326794967 -0.842128773015309
-0.929796326794967 -0.841328917898403
-0.928796326794967 -0.840530367653027
-0.927796326794967 -0.83973311851142
-0.926796326794967 -0.838937166716669
-0.925796326794968 -0.838142508522682
-0.924796326794968 -0.837349140194168
-0.923796326794968 -0.836557058006605
-0.922796326794968 -0.835766258246218
-0.921796326794968 -0.834976737209955
-0.920796326794968 -0.83418849120546
-0.919796326794968 -0.833401516551045
-0.918796326794968 -0.832615809575669
-0.917796326794968 -0.831831366618909
-0.916796326794969 -0.831048184030938
-0.915796326794969 -0.830266258172492
-0.914796326794969 -0.829485585414853
-0.913796326794969 -0.828706162139818
-0.912796326794969 -0.827927984739673
-0.911796326794969 -0.827151049617169
-0.910796326794969 -0.826375353185497
-0.909796326794969 -0.825600891868256
-0.908796326794969 -0.824827662099436
-0.90779632679497 -0.824055660323383
-0.90679632679497 -0.823284882994781
-0.90579632679497 -0.822515326578617
-0.90479632679497 -0.821746987550164
-0.90379632679497 -0.820979862394948
-0.90279632679497 -0.820213947608724
-0.90179632679497 -0.819449239697452
-0.90079632679497 -0.818685735177266
-0.89979632679497 -0.817923430574451
-0.898796326794971 -0.817162322425417
-0.897796326794971 -0.816402407276669
-0.896796326794971 -0.815643681684784
-0.895796326794971 -0.814886142216386
-0.894796326794971 -0.814129785448113
-0.893796326794971 -0.813374607966598
-0.892796326794971 -0.812620606368438
-0.891796326794971 -0.811867777260168
};
\addplot [semithick, blue]
table {%
-0.890796326794971 -0.729367287018002
-0.889796326794972 -0.728927625290068
-0.888796326794972 -0.728489045227928
-0.887796326794972 -0.728051542138952
-0.886796326794972 -0.727615111356173
-0.885796326794972 -0.727179748238121
-0.884796326794972 -0.726745448168647
-0.883796326794972 -0.726312206556757
-0.882796326794972 -0.725880018836439
-0.881796326794972 -0.725448880466501
-0.880796326794973 -0.725018786930403
-0.879796326794973 -0.724589733736092
-0.878796326794973 -0.724161716415839
-0.877796326794973 -0.723734730526079
-0.876796326794973 -0.723308771647247
-0.875796326794973 -0.72288383538362
-0.874796326794973 -0.722459917363162
-0.873796326794973 -0.72203701323736
-0.872796326794973 -0.721615118681076
-0.871796326794974 -0.721194229392387
-0.870796326794974 -0.720774341092432
-0.869796326794974 -0.720355449525263
-0.868796326794974 -0.719937550457691
-0.867796326794974 -0.719520639679138
-0.866796326794974 -0.719104713001485
-0.865796326794974 -0.718689766258929
-0.864796326794974 -0.718275795307833
-0.863796326794974 -0.717862796026582
-0.862796326794975 -0.717450764315438
-0.861796326794975 -0.717039696096398
-0.860796326794975 -0.716629587313051
-0.859796326794975 -0.716220433930436
-0.858796326794975 -0.715812231934906
-0.857796326794975 -0.715404977333983
-0.856796326794975 -0.714998666156226
-0.855796326794975 -0.71459329445109
-0.854796326794975 -0.714188858288795
-0.853796326794976 -0.713785353760183
-0.852796326794976 -0.713382776976594
-0.851796326794976 -0.712981124069727
-0.850796326794976 -0.712580391191512
-0.849796326794976 -0.712180574513975
-0.848796326794976 -0.71178167022911
-0.847796326794976 -0.711383674548755
-0.846796326794976 -0.710986583704457
-0.845796326794976 -0.710590393947349
-0.844796326794977 -0.710195101548022
-0.843796326794977 -0.709800702796404
-0.842796326794977 -0.709407194001633
-0.841796326794977 -0.709014571491931
-0.840796326794977 -0.708622831614491
-0.839796326794977 -0.708231970735345
-0.838796326794977 -0.70784198523925
-0.837796326794977 -0.707452871529568
-0.836796326794977 -0.707064626028146
-0.835796326794978 -0.706677245175198
-0.834796326794978 -0.70629072542919
-0.833796326794978 -0.705905063266724
-0.832796326794978 -0.705520255182419
-0.831796326794978 -0.705136297688802
-0.830796326794978 -0.704753187316193
-0.829796326794978 -0.704370920612588
-0.828796326794978 -0.703989494143555
-0.827796326794978 -0.703608904492118
-0.826796326794978 -0.703229148258645
-0.825796326794979 -0.702850222060746
-0.824796326794979 -0.702472122533158
-0.823796326794979 -0.702094846327639
-0.822796326794979 -0.701718390112863
-0.821796326794979 -0.70134275057431
-0.820796326794979 -0.700967924414164
-0.819796326794979 -0.700593908351211
-0.818796326794979 -0.700220699120727
-0.817796326794979 -0.69984829347438
-0.81679632679498 -0.699476688180131
-0.81579632679498 -0.699105880022124
-0.81479632679498 -0.698735865800593
-0.81379632679498 -0.698366642331758
-0.81279632679498 -0.697998206447725
-0.81179632679498 -0.697630554996391
-0.81079632679498 -0.697263684841343
-0.80979632679498 -0.69689759286176
-0.80879632679498 -0.69653227595232
-0.807796326794981 -0.6961677310231
-0.806796326794981 -0.695803954999485
-0.805796326794981 -0.695440944822072
-0.804796326794981 -0.695078697446574
-0.803796326794981 -0.69471720984373
-0.802796326794981 -0.694356478999208
-0.801796326794981 -0.693996501913521
-0.800796326794981 -0.69363727560193
-0.799796326794981 -0.693278797094353
-0.798796326794982 -0.692921063435278
-0.797796326794982 -0.692564071683675
-0.796796326794982 -0.692207818912901
-0.795796326794982 -0.69185230221062
-0.794796326794982 -0.69149751867871
-0.793796326794982 -0.691143465433181
-0.792796326794982 -0.690790139604084
-0.791796326794982 -0.690437538335429
-0.790796326794982 -0.690085658785098
-0.789796326794983 -0.689734498124764
-0.788796326794983 -0.689384053539803
-0.787796326794983 -0.689034322229215
-0.786796326794983 -0.688685301405538
-0.785796326794983 -0.68833698829477
-0.784796326794983 -0.687989380136285
-0.783796326794983 -0.68764247418275
-0.782796326794983 -0.687296267700052
-0.781796326794983 -0.686950757967212
-0.780796326794984 -0.686605942276308
-0.779796326794984 -0.686261817932396
-0.778796326794984 -0.685918382253435
-0.777796326794984 -0.685575632570205
-0.776796326794984 -0.685233566226232
-0.775796326794984 -0.684892180577716
-0.774796326794984 -0.684551472993446
-0.773796326794984 -0.684211440854735
};
\addplot [semithick, blue]
table {%
-0.772796326794984 -0.610049635712001
-0.771796326794985 -0.610195290150481
-0.770796326794985 -0.610340545031978
-0.769796326794985 -0.610485402281541
-0.768796326794985 -0.610629863812174
-0.767796326794985 -0.610773931524932
-0.766796326794985 -0.610917607309012
-0.765796326794985 -0.611060893041849
-0.764796326794985 -0.611203790589205
-0.763796326794985 -0.611346301805262
-0.762796326794986 -0.61148842853271
-0.761796326794986 -0.611630172602839
-0.760796326794986 -0.611771535835628
-0.759796326794986 -0.611912520039826
-0.758796326794986 -0.612053127013047
-0.757796326794986 -0.612193358541854
-0.756796326794986 -0.61233321640184
-0.755796326794986 -0.612472702357719
-0.754796326794986 -0.612611818163403
-0.753796326794987 -0.612750565562092
-0.752796326794987 -0.612888946286349
-0.751796326794987 -0.613026962058186
-0.750796326794987 -0.613164614589145
-0.749796326794987 -0.613301905580376
-0.748796326794987 -0.613438836722717
-0.747796326794987 -0.61357540969677
-0.746796326794987 -0.613711626172985
-0.745796326794987 -0.61384748781173
-0.744796326794988 -0.613982996263373
-0.743796326794988 -0.614118153168353
-0.742796326794988 -0.614252960157261
-0.741796326794988 -0.614387418850905
-0.740796326794988 -0.614521530860394
-0.739796326794988 -0.614655297787204
-0.738796326794988 -0.614788721223256
-0.737796326794988 -0.61492180275098
-0.736796326794988 -0.615054543943393
-0.735796326794989 -0.615186946364166
-0.734796326794989 -0.615319011567695
-0.733796326794989 -0.615450741099171
-0.732796326794989 -0.615582136494645
-0.731796326794989 -0.6157131992811
-0.730796326794989 -0.615843930976517
-0.729796326794989 -0.61597433308994
-0.728796326794989 -0.616104407121544
-0.727796326794989 -0.616234154562702
-0.72679632679499 -0.616363576896047
-0.72579632679499 -0.616492675595536
-0.72479632679499 -0.616621452126518
-0.72379632679499 -0.616749907945793
-0.72279632679499 -0.616878044501678
-0.72179632679499 -0.617005863234066
-0.72079632679499 -0.617133365574492
-0.71979632679499 -0.617260552946188
-0.71879632679499 -0.617387426764149
-0.717796326794991 -0.617513988435192
-0.716796326794991 -0.617640239358012
-0.715796326794991 -0.617766180923247
-0.714796326794991 -0.617891814513529
-0.713796326794991 -0.61801714150355
-0.712796326794991 -0.618142163260113
-0.711796326794991 -0.618266881142194
-0.710796326794991 -0.618391296500992
-0.709796326794991 -0.618515410679995
-0.708796326794991 -0.618639225015024
-0.707796326794992 -0.618762740834297
-0.706796326794992 -0.618885959458479
-0.705796326794992 -0.619008882200739
-0.704796326794992 -0.619131510366801
-0.703796326794992 -0.619253845254996
-0.702796326794992 -0.619375888156322
-0.701796326794992 -0.619497640354486
};
\addplot [semithick, blue]
table {%
-0.700796326794992 -0.555434510884232
-0.699796326794992 -0.556175785838315
-0.698796326794993 -0.556914796646977
-0.697796326794993 -0.557651554335536
-0.696796326794993 -0.558386069862984
-0.695796326794993 -0.559118354122449
-0.694796326794993 -0.559848417941651
-0.693796326794993 -0.560576272083357
-0.692796326794993 -0.561301927245839
-0.691796326794993 -0.562025394063314
-0.690796326794993 -0.562746683106393
-0.689796326794994 -0.563465804882526
-0.688796326794994 -0.564182769836435
-0.687796326794994 -0.56489758835055
-0.686796326794994 -0.565610270745445
-0.685796326794994 -0.566320827280263
-0.684796326794994 -0.567029268153143
-0.683796326794994 -0.567735603501643
-0.682796326794994 -0.568439843403156
-0.681796326794994 -0.569141997875332
-0.680796326794995 -0.569842076876485
-0.679796326794995 -0.570540090306005
-0.678796326794995 -0.571236048004768
-0.677796326794995 -0.571929959755536
-0.676796326794995 -0.572621835283358
-0.675796326794995 -0.573311684255971
-0.674796326794995 -0.573999516284189
-0.673796326794995 -0.574685340922304
-0.672796326794995 -0.575369167668465
-0.671796326794996 -0.576051005965071
-0.670796326794996 -0.576730865199151
-0.669796326794996 -0.577408754702746
-0.668796326794996 -0.578084683753286
-0.667796326794996 -0.578758661573962
-0.666796326794996 -0.579430697334103
-0.665796326794996 -0.58010080014954
-0.664796326794996 -0.580768979082978
-0.663796326794996 -0.581435243144353
-0.662796326794997 -0.582099601291198
-0.661796326794997 -0.582762062428997
-0.660796326794997 -0.583422635411546
-0.659796326794997 -0.5840813290413
-0.658796326794997 -0.584738152069727
-0.657796326794997 -0.585393113197656
-0.656796326794997 -0.586046221075617
-0.655796326794997 -0.586697484304189
-0.654796326794997 -0.587346911434339
-0.653796326794998 -0.587994510967754
-0.652796326794998 -0.588640291357183
};
\addplot [semithick, blue]
table {%
-0.651796326794998 -0.534234258251982
-0.650796326794998 -0.535626731857043
-0.649796326794998 -0.53701440928619
-0.648796326794998 -0.53839731272064
-0.647796326794998 -0.539775464243261
-0.646796326794998 -0.541148885838682
-0.645796326794998 -0.542517599393408
-0.644796326794999 -0.54388162669594
-0.643796326794999 -0.545240989436906
-0.642796326794999 -0.546595709209203
-0.641796326794999 -0.547945807508134
-0.640796326794999 -0.549291305731566
-0.639796326794999 -0.550632225180085
-0.638796326794999 -0.551968587057161
-0.637796326794999 -0.553300412469323
-0.636796326794999 -0.554627722426332
-0.635796326795 -0.55595053784137
-0.634796326795 -0.557268879531225
-0.633796326795 -0.558582768216491
-0.632796326795 -0.559892224521769
-0.631796326795 -0.56119726897587
-0.630796326795 -0.562497922012034
-0.629796326795 -0.563794203968142
-0.628796326795 -0.565086135086941
-0.627796326795 -0.566373735516274
-0.626796326795001 -0.567657025309308
-0.625796326795001 -0.568936024424774
-0.624796326795001 -0.570210752727209
-0.623796326795001 -0.571481229987202
-0.622796326795001 -0.572747475881642
-0.621796326795001 -0.574009509993977
-0.620796326795001 -0.57526735181447
-0.619796326795001 -0.576521020740458
-0.618796326795001 -0.577770536076628
-0.617796326795002 -0.579015917035278
-0.616796326795002 -0.580257182736594
-0.615796326795002 -0.581494352208928
};
\addplot [semithick, blue]
table {%
-0.614796326795002 -0.537550513368968
-0.613796326795002 -0.539659772211928
-0.612796326795002 -0.54176068881294
-0.611796326795002 -0.543853298305755
-0.610796326795002 -0.545937635804756
-0.609796326795002 -0.54801373640181
-0.608796326795003 -0.550081635163188
-0.607796326795003 -0.552141367126552
-0.606796326795003 -0.554192967298007
-0.605796326795003 -0.556236470649221
-0.604796326795003 -0.558271912114605
-0.603796326795003 -0.560299326588564
-0.602796326795003 -0.562318748922801
-0.601796326795003 -0.56433021392369
-0.600796326795003 -0.566333756349702
-0.599796326795003 -0.568329410908906
-0.598796326795004 -0.570317212256511
-0.597796326795004 -0.572297194992477
-0.596796326795004 -0.57426939365918
-0.595796326795004 -0.576233842739136
-0.594796326795004 -0.578190576652779
-0.593796326795004 -0.580139629756289
-0.592796326795004 -0.582081036339485
-0.591796326795004 -0.58401483062376
-0.590796326795004 -0.585941046760077
-0.589796326795005 -0.587859718827009
-0.588796326795005 -0.589770880828832
-0.587796326795005 -0.591674566693676
-0.586796326795005 -0.593570810271712
-0.585796326795005 -0.595459645333393
};
\addplot [semithick, blue]
table {%
-0.584796326795005 -0.563823763384451
-0.583796326795005 -0.566703039551792
-0.582796326795005 -0.56956889882895
-0.581796326795005 -0.572421393722459
-0.580796326795006 -0.575260577067031
-0.579796326795006 -0.578086502010858
-0.578796326795006 -0.580899222001171
-0.577796326795006 -0.583698790770075
-0.576796326795006 -0.586485262320629
-0.575796326795006 -0.589258690913204
-0.574796326795006 -0.592019131052081
-0.573796326795006 -0.594766637472314
-0.572796326795006 -0.597501265126839
-0.571796326795007 -0.600223069173847
-0.570796326795007 -0.602932104964392
-0.569796326795007 -0.605628428030248
-0.568796326795007 -0.608312094072011
-0.567796326795007 -0.61098315894745
-0.566796326795007 -0.613641678660079
-0.565796326795007 -0.616287709347987
-0.564796326795007 -0.618921307272875
-0.563796326795007 -0.621542528809359
-0.562796326795008 -0.624151430434463
-0.561796326795008 -0.626748068717367
-0.560796326795008 -0.629332500309365
-0.559796326795008 -0.631904781934043
-0.558796326795008 -0.634464970377681
};
\addplot [semithick, blue]
table {%
-0.557796326795008 -0.619237125509078
-0.556796326795008 -0.622870719425163
-0.555796326795008 -0.626483718272454
-0.554796326795008 -0.630076210291385
-0.553796326795009 -0.633648284759322
-0.552796326795009 -0.637200031944736
-0.551796326795009 -0.640731543062272
-0.550796326795009 -0.644242910228705
-0.549796326795009 -0.647734226419813
-0.548796326795009 -0.651205585428126
-0.547796326795009 -0.65465708182155
-0.546796326795009 -0.658088810902899
-0.545796326795009 -0.661500868670265
-0.54479632679501 -0.664893351778282
-0.54379632679501 -0.668266357500235
-0.54279632679501 -0.671619983691023
-0.54179632679501 -0.674954328750964
-0.54079632679501 -0.678269491590444
-0.53979632679501 -0.681565571595383
-0.53879632679501 -0.68484266859352
-0.53779632679501 -0.688100882821516
-0.53679632679501 -0.691340314892842
-0.535796326795011 -0.694561065766469
-0.534796326795011 -0.697763236716334
-0.533796326795011 -0.700946929301565
-0.532796326795011 -0.704112245337489
-0.531796326795011 -0.707259286867361
-0.530796326795011 -0.71038815613485
-0.529796326795011 -0.713498955557247
-0.528796326795011 -0.716591787699387
-0.527796326795011 -0.719666755248276
-0.526796326795012 -0.72272396098842
-0.525796326795012 -0.725763507777941
-0.524796326795012 -0.728785498524931
-0.523796326795012 -0.731790036165097
-0.522796326795012 -0.734777223639665
-0.521796326795012 -0.737747163873999
-0.520796326795012 -0.740699959756861
-0.519796326795012 -0.743635714120276
-0.518796326795012 -0.746554529720008
-0.517796326795013 -0.749456509216635
-0.516796326795013 -0.752341755157192
-0.515796326795013 -0.7552103699574
-0.514796326795013 -0.758062455884442
-0.513796326795013 -0.760898115040303
-0.512796326795013 -0.763717449345633
-0.511796326795013 -0.766520560524142
-0.510796326795013 -0.769307550087525
-0.509796326795013 -0.772078519320867
-0.508796326795014 -0.774833569268569
-0.507796326795014 -0.777572800720743
-0.506796326795014 -0.780296314200083
-0.505796326795014 -0.783004209949209
-0.504796326795014 -0.785696587918453
-0.503796326795014 -0.788373547754102
-0.502796326795014 -0.791035188787056
-0.501796326795014 -0.793681610021934
-0.500796326795014 -0.796312910126574
-0.499796326795015 -0.79892918742195
-0.498796326795015 -0.801530539872477
-0.497796326795015 -0.804117065076706
};
\addplot [semithick, blue]
table {%
-0.496796326795015 -0.771920248063213
-0.495796326795015 -0.773830661551888
-0.494796326795015 -0.775732445104288
-0.493796326795015 -0.777625647178825
-0.492796326795015 -0.779510316009477
-0.491796326795015 -0.78138649960489
-0.490796326795016 -0.783254245747565
-0.489796326795016 -0.785113601993072
-0.488796326795016 -0.786964615669345
-0.487796326795016 -0.788807333876026
-0.486796326795016 -0.790641803483857
-0.485796326795016 -0.79246807113413
-0.484796326795016 -0.794286183238192
-0.483796326795016 -0.796096185976992
-0.482796326795016 -0.797898125300684
-0.481796326795016 -0.799692046928275
-0.480796326795017 -0.80147799634732
-0.479796326795017 -0.80325601881366
-0.478796326795017 -0.80502615935121
-0.477796326795017 -0.806788462751784
-0.476796326795017 -0.808542973574961
-0.475796326795017 -0.810289736148004
-0.474796326795017 -0.8120287945658
-0.473796326795017 -0.813760192690853
-0.472796326795017 -0.81548397415331
-0.471796326795018 -0.817200182351021
-0.470796326795018 -0.818908860449638
-0.469796326795018 -0.820610051382747
-0.468796326795018 -0.822303797852035
};
\addplot [semithick, blue]
table {%
-0.467796326795018 -0.774924176335164
-0.466796326795018 -0.776141637061213
-0.465796326795018 -0.777354940214148
-0.464796326795018 -0.778564105914772
-0.463796326795018 -0.7797691541788
-0.462796326795019 -0.780970104917279
-0.461796326795019 -0.782166977937028
-0.460796326795019 -0.783359792941065
-0.459796326795019 -0.784548569529039
-0.458796326795019 -0.785733327197669
-0.457796326795019 -0.786914085341181
-0.456796326795019 -0.788090863251741
-0.455796326795019 -0.789263680119903
-0.454796326795019 -0.790432555035039
-0.45379632679502 -0.791597506985788
-0.45279632679502 -0.792758554860498
-0.45179632679502 -0.793915717447665
-0.45079632679502 -0.795069013436383
-0.44979632679502 -0.796218461416786
-0.44879632679502 -0.797364079880493
-0.44779632679502 -0.798505887221057
-0.44679632679502 -0.799643901734411
-0.44579632679502 -0.800778141619315
-0.444796326795021 -0.801908624977805
-0.443796326795021 -0.80303536981564
-0.442796326795021 -0.804158394042751
-0.441796326795021 -0.805277715473692
-0.440796326795021 -0.806393351828083
-0.439796326795021 -0.807505320731067
-0.438796326795021 -0.808613639713752
-0.437796326795021 -0.809718326213666
-0.436796326795021 -0.8108193975752
-0.435796326795022 -0.811916871050062
-0.434796326795022 -0.813010763797724
};
\addplot [semithick, blue]
table {%
-0.433796326795022 -0.754107564046463
-0.432796326795022 -0.75483573444583
-0.431796326795022 -0.755562086817781
-0.430796326795022 -0.756286628646155
-0.429796326795022 -0.757009367377907
-0.428796326795022 -0.757730310423317
-0.427796326795022 -0.758449465156187
-0.426796326795023 -0.759166838914049
-0.425796326795023 -0.759882438998359
-0.424796326795023 -0.760596272674705
-0.423796326795023 -0.761308347173003
-0.422796326795023 -0.762018669687692
-0.421796326795023 -0.762727247377937
-0.420796326795023 -0.763434087367816
-0.419796326795023 -0.764139196746524
-0.418796326795023 -0.764842582568561
-0.417796326795024 -0.765544251853926
-0.416796326795024 -0.766244211588309
-0.415796326795024 -0.766942468723277
-0.414796326795024 -0.767639030176472
-0.413796326795024 -0.768333902831791
-0.412796326795024 -0.769027093539577
-0.411796326795024 -0.769718609116805
-0.410796326795024 -0.770408456347267
-0.409796326795024 -0.771096641981754
-0.408796326795025 -0.771783172738243
-0.407796326795025 -0.772468055302075
-0.406796326795025 -0.773151296326138
-0.405796326795025 -0.773832902431048
-0.404796326795025 -0.774512880205324
-0.403796326795025 -0.77519123620557
-0.402796326795025 -0.775867976956652
-0.401796326795025 -0.77654310895187
-0.400796326795025 -0.777216638653135
-0.399796326795026 -0.777888572491146
-0.398796326795026 -0.778558916865558
-0.397796326795026 -0.779227678145156
-0.396796326795026 -0.779894862668026
-0.395796326795026 -0.780560476741727
-0.394796326795026 -0.781224526643455
-0.393796326795026 -0.781887018620217
-0.392796326795026 -0.782547958888994
-0.391796326795026 -0.783207353636908
-0.390796326795027 -0.783865209021389
};
\addplot [semithick, blue]
table {%
-0.389796326795027 -0.71397712862076
-0.388796326795027 -0.714335353282407
-0.387796326795027 -0.714692957320007
-0.386796326795027 -0.715049942967141
-0.385796326795027 -0.715406312447828
-0.384796326795027 -0.715762067976589
-0.383796326795027 -0.716117211758484
-0.382796326795027 -0.716471745989176
-0.381796326795028 -0.716825672854972
-0.380796326795028 -0.717178994532882
-0.379796326795028 -0.717531713190663
-0.378796326795028 -0.717883830986869
-0.377796326795028 -0.718235350070906
-0.376796326795028 -0.718586272583077
-0.375796326795028 -0.718936600654631
-0.374796326795028 -0.719286336407813
-0.373796326795028 -0.719635481955912
-0.372796326795028 -0.71998403940331
-0.371796326795029 -0.720332010845528
-0.370796326795029 -0.720679398369274
-0.369796326795029 -0.721026204052492
-0.368796326795029 -0.721372429964405
-0.367796326795029 -0.721718078165566
-0.366796326795029 -0.722063150707903
-0.365796326795029 -0.722407649634763
-0.364796326795029 -0.72275157698096
-0.363796326795029 -0.72309493477282
-0.36279632679503 -0.723437725028225
-0.36179632679503 -0.723779949756659
-0.36079632679503 -0.724121610959254
-0.35979632679503 -0.724462710628832
-0.35879632679503 -0.724803250749949
-0.35779632679503 -0.725143233298942
-0.35679632679503 -0.725482660243969
-0.35579632679503 -0.725821533545053
-0.35479632679503 -0.726159855154129
-0.353796326795031 -0.726497627015079
-0.352796326795031 -0.726834851063784
-0.351796326795031 -0.727171529228159
-0.350796326795031 -0.727507663428195
-0.349796326795031 -0.727843255576008
-0.348796326795031 -0.728178307575873
-0.347796326795031 -0.728512821324267
-0.346796326795031 -0.728846798709912
-0.345796326795031 -0.729180241613816
-0.344796326795032 -0.729513151909311
-0.343796326795032 -0.729845531462092
-0.342796326795032 -0.730177382130264
-0.341796326795032 -0.730508705764374
-0.340796326795032 -0.730839504207455
-0.339796326795032 -0.731169779295063
-0.338796326795032 -0.731499532855319
-0.337796326795032 -0.731828766708945
-0.336796326795032 -0.732157482669301
-0.335796326795033 -0.732485682542431
-0.334796326795033 -0.732813368127092
-0.333796326795033 -0.733140541214797
-0.332796326795033 -0.733467203589853
-0.331796326795033 -0.733793357029396
-0.330796326795033 -0.734119003303428
-0.329796326795033 -0.734444144174858
-0.328796326795033 -0.734768781399534
-0.327796326795033 -0.735092916726284
-0.326796326795034 -0.735416551896947
};
\addplot [semithick, blue]
table {%
-0.325796326795034 -0.65214940526605
-0.324796326795034 -0.652214366108601
-0.323796326795034 -0.652279256587774
-0.322796326795034 -0.652344076946854
-0.321796326795034 -0.652408827428323
-0.320796326795034 -0.652473508273865
-0.319796326795034 -0.652538119724368
-0.318796326795034 -0.652602662019927
-0.317796326795035 -0.65266713539985
-0.316796326795035 -0.652731540102664
-0.315796326795035 -0.652795876366111
-0.314796326795035 -0.65286014442716
-0.313796326795035 -0.652924344522008
-0.312796326795035 -0.652988476886081
-0.311796326795035 -0.653052541754042
-0.310796326795035 -0.653116539359792
-0.309796326795035 -0.653180469936475
-0.308796326795036 -0.65324433371648
-0.307796326795036 -0.653308130931448
-0.306796326795036 -0.653371861812272
-0.305796326795036 -0.653435526589103
-0.304796326795036 -0.653499125491352
-0.303796326795036 -0.653562658747695
-0.302796326795036 -0.653626126586075
-0.301796326795036 -0.653689529233709
-0.300796326795036 -0.653752866917086
-0.299796326795037 -0.653816139861976
-0.298796326795037 -0.653879348293429
-0.297796326795037 -0.653942492435783
-0.296796326795037 -0.654005572512663
-0.295796326795037 -0.654068588746988
-0.294796326795037 -0.65413154136097
-0.293796326795037 -0.654194430576125
-0.292796326795037 -0.654257256613268
-0.291796326795037 -0.654320019692522
-0.290796326795038 -0.654382720033317
-0.289796326795038 -0.6544453578544
-0.288796326795038 -0.654507933373829
-0.287796326795038 -0.654570446808987
-0.286796326795038 -0.654632898376574
-0.285796326795038 -0.654695288292621
-0.284796326795038 -0.654757616772485
-0.283796326795038 -0.654819884030857
-0.282796326795038 -0.654882090281762
-0.281796326795039 -0.654944235738567
-0.280796326795039 -0.655006320613977
-0.279796326795039 -0.655068345120047
-0.278796326795039 -0.655130309468177
-0.277796326795039 -0.655192213869118
-0.276796326795039 -0.65525405853298
-0.275796326795039 -0.655315843669225
-0.274796326795039 -0.655377569486681
-0.273796326795039 -0.655439236193537
-0.27279632679504 -0.655500843997351
-0.27179632679504 -0.655562393105049
-0.27079632679504 -0.65562388372293
-0.26979632679504 -0.655685316056673
-0.26879632679504 -0.655746690311331
-0.26779632679504 -0.655808006691342
-0.26679632679504 -0.65586926540053
-0.26579632679504 -0.655930466642103
-0.26479632679504 -0.655991610618665
-0.263796326795041 -0.65605269753221
-0.262796326795041 -0.65611372758413
-0.261796326795041 -0.656174700975219
-0.260796326795041 -0.656235617905669
-0.259796326795041 -0.656296478575082
-0.258796326795041 -0.656357283182466
-0.257796326795041 -0.656418031926239
-0.256796326795041 -0.656478725004236
-0.255796326795041 -0.656539362613707
-0.254796326795041 -0.656599944951321
-0.253796326795042 -0.656660472213171
-0.252796326795042 -0.656720944594775
-0.251796326795042 -0.656781362291076
-0.250796326795042 -0.656841725496452
-0.249796326795042 -0.656902034404712
-0.248796326795042 -0.6569622892091
-0.247796326795042 -0.6570224901023
-0.246796326795042 -0.65708263727644
-0.245796326795042 -0.657142730923087
-0.244796326795043 -0.657202771233259
-0.243796326795043 -0.657262758397421
-0.242796326795043 -0.657322692605491
-0.241796326795043 -0.657382574046844
-0.240796326795043 -0.657442402910307
-0.239796326795043 -0.657502179384172
-0.238796326795043 -0.65756190365619
-0.237796326795043 -0.657621575913581
-0.236796326795043 -0.657681196343027
-0.235796326795044 -0.657740765130687
-0.234796326795044 -0.657800282462186
-0.233796326795044 -0.657859748522629
-0.232796326795044 -0.657919163496598
-0.231796326795044 -0.657978527568152
};
\addplot [semithick, blue]
table {%
-0.230796326795044 -0.556591930757097
-0.229796326795044 -0.556413371532235
-0.228796326795044 -0.556234906563391
-0.227796326795044 -0.556056535430665
-0.226796326795045 -0.555878257714947
-0.225796326795045 -0.555700072997917
-0.224796326795045 -0.555521980862039
-0.223796326795045 -0.555343980890559
-0.222796326795045 -0.555166072667497
-0.221796326795045 -0.554988255777646
-0.220796326795045 -0.554810529806569
-0.219796326795045 -0.554632894340591
-0.218796326795045 -0.554455348966798
-0.217796326795046 -0.554277893273032
-0.216796326795046 -0.554100526847887
-0.215796326795046 -0.553923249280707
-0.214796326795046 -0.553746060161578
-0.213796326795046 -0.553568959081328
-0.212796326795046 -0.55339194563152
-0.211796326795046 -0.55321501940445
-0.210796326795046 -0.553038179993143
-0.209796326795046 -0.552861426991349
-0.208796326795047 -0.552684759993537
-0.207796326795047 -0.552508178594895
-0.206796326795047 -0.552331682391322
-0.205796326795047 -0.55215527097943
-0.204796326795047 -0.551978943956531
-0.203796326795047 -0.551802700920642
-0.202796326795047 -0.551626541470478
-0.201796326795047 -0.551450465205447
-0.200796326795047 -0.551274471725646
-0.199796326795048 -0.551098560631861
-0.198796326795048 -0.55092273152556
-0.197796326795048 -0.550746984008887
-0.196796326795048 -0.550571317684665
-0.195796326795048 -0.550395732156387
-0.194796326795048 -0.550220227028214
-0.193796326795048 -0.55004480190497
-0.192796326795048 -0.549869456392141
-0.191796326795048 -0.549694190095868
-0.190796326795049 -0.549519002622946
-0.189796326795049 -0.54934389358082
-0.188796326795049 -0.54916886257758
-0.187796326795049 -0.548993909221958
-0.186796326795049 -0.548819033123325
-0.185796326795049 -0.548644233891686
-0.184796326795049 -0.548469511137679
-0.183796326795049 -0.548294864472568
-0.182796326795049 -0.548120293508241
-0.18179632679505 -0.547945797857209
-0.18079632679505 -0.547771377132598
-0.17979632679505 -0.547597030948148
-0.17879632679505 -0.547422758918209
-0.17779632679505 -0.547248560657737
-0.17679632679505 -0.547074435782292
-0.17579632679505 -0.546900383908032
-0.17479632679505 -0.546726404651714
-0.17379632679505 -0.546552497630682
-0.172796326795051 -0.546378662462875
-0.171796326795051 -0.546204898766814
-0.170796326795051 -0.546031206161604
-0.169796326795051 -0.545857584266926
-0.168796326795051 -0.545684032703039
-0.167796326795051 -0.545510551090773
-0.166796326795051 -0.545337139051526
-0.165796326795051 -0.545163796207262
-0.164796326795051 -0.544990522180505
-0.163796326795052 -0.54481731659434
-0.162796326795052 -0.544644179072403
-0.161796326795052 -0.544471109238886
-0.160796326795052 -0.544298106718525
-0.159796326795052 -0.544125171136605
-0.158796326795052 -0.543952302118949
-0.157796326795052 -0.543779499291921
-0.156796326795052 -0.543606762282417
-0.155796326795052 -0.543434090717867
-0.154796326795053 -0.543261484226229
-0.153796326795053 -0.543088942435986
-0.152796326795053 -0.542916464976141
-0.151796326795053 -0.542744051476218
-0.150796326795053 -0.542571701566254
-0.149796326795053 -0.542399414876801
-0.148796326795053 -0.542227191038916
-0.147796326795053 -0.542055029684165
-0.146796326795053 -0.541882930444615
-0.145796326795053 -0.54171089295283
-0.144796326795054 -0.541538916841874
-0.143796326795054 -0.5413670017453
-0.142796326795054 -0.541195147297152
-0.141796326795054 -0.541023353131961
-0.140796326795054 -0.540851618884741
-0.139796326795054 -0.540679944190985
-0.138796326795054 -0.540508328686663
-0.137796326795054 -0.54033677200822
-0.136796326795054 -0.540165273792569
-0.135796326795055 -0.539993833677094
-0.134796326795055 -0.539822451299641
-0.133796326795055 -0.539651126298517
-0.132796326795055 -0.539479858312489
-0.131796326795055 -0.539308646980776
-0.130796326795055 -0.539137491943051
-0.129796326795055 -0.538966392839436
-0.128796326795055 -0.538795349310499
-0.127796326795055 -0.538624360997248
-0.126796326795056 -0.538453427541133
-0.125796326795056 -0.538282548584042
-0.124796326795056 -0.538111723768292
-0.123796326795056 -0.537940952736634
-0.122796326795056 -0.537770235132246
-0.121796326795056 -0.53759957059873
-0.120796326795056 -0.537428958780108
-0.119796326795056 -0.537258399320823
-0.118796326795056 -0.537087891865732
-0.117796326795057 -0.536917436060104
-0.116796326795057 -0.536747031549618
-0.115796326795057 -0.536576677980359
-0.114796326795057 -0.536406374998817
-0.113796326795057 -0.53623612225188
-0.112796326795057 -0.536065919386836
-0.111796326795057 -0.535895766051365
-0.110796326795057 -0.535725661893541
-0.109796326795057 -0.535555606561825
-0.108796326795058 -0.535385599705065
-0.107796326795058 -0.535215640972491
-0.106796326795058 -0.535045730013713
-0.105796326795058 -0.534875866478718
-0.104796326795058 -0.534706050017866
-0.103796326795058 -0.534536280281891
-0.102796326795058 -0.534366556921893
-0.101796326795058 -0.534196879589337
-0.100796326795058 -0.534027247936052
-0.0997963267950586 -0.533857661614226
-0.0987963267950587 -0.533688120276403
-0.0977963267950588 -0.533518623575483
-0.0967963267950589 -0.533349171164714
-0.095796326795059 -0.533179762697693
-0.0947963267950591 -0.533010397828365
-0.0937963267950592 -0.532841076211015
-0.0927963267950593 -0.532671797500266
-0.0917963267950594 -0.532502560854369
-0.0907963267950596 -0.532333366304314
-0.0897963267950597 -0.532164214380953
-0.0887963267950598 -0.531995103824704
-0.0877963267950599 -0.531826035057327
-0.08679632679506 -0.531657006520448
-0.0857963267950601 -0.531488018485562
-0.0847963267950602 -0.53131907060955
-0.0837963267950603 -0.531150162549634
-0.0827963267950604 -0.530981293963381
-0.0817963267950605 -0.530812464508696
-0.0807963267950607 -0.530643673843822
-0.0797963267950608 -0.530474921627342
-0.0787963267950609 -0.530306207518175
-0.077796326795061 -0.530137531175578
-0.0767963267950611 -0.529968892259144
-0.0757963267950612 -0.529800290428802
-0.0747963267950613 -0.529631725344819
-0.0737963267950614 -0.529463196667804
-0.0727963267950615 -0.529294704058703
};
\addplot [semithick, blue]
table {%
-0.0717963267950616 -0.397472614189643
-0.0707963267950618 -0.397069477654869
-0.0697963267950619 -0.396666353809191
-0.068796326795062 -0.396263241977196
-0.0677963267950621 -0.395860141483625
-0.0667963267950622 -0.39545705165338
-0.0657963267950623 -0.39505397181153
-0.0647963267950624 -0.394650901283317
-0.0637963267950625 -0.394247839387811
-0.0627963267950626 -0.393844785424642
-0.0617963267950628 -0.393441738743558
-0.0607963267950629 -0.393038698669233
-0.059796326795063 -0.392635664526383
-0.0587963267950631 -0.392232635639757
-0.0577963267950632 -0.391829611301034
-0.0567963267950633 -0.391426590893137
-0.0557963267950634 -0.391023573716017
-0.0547963267950635 -0.390620559094524
-0.0537963267950636 -0.390217546353524
-0.0527963267950637 -0.389814534817891
-0.0517963267950639 -0.389411523812511
-0.050796326795064 -0.389008512662271
-0.0497963267950641 -0.388605500692056
-0.0487963267950642 -0.388202487226749
-0.0477963267950643 -0.387799471591222
-0.0467963267950644 -0.387396453110334
-0.0457963267950645 -0.386993431108928
-0.0447963267950646 -0.386590404911826
-0.0437963267950647 -0.386187373843822
-0.0427963267950648 -0.385784337229684
-0.041796326795065 -0.385381294394145
-0.0407963267950651 -0.384978244661899
-0.0397963267950652 -0.384575187357602
-0.0387963267950653 -0.38417212180586
-0.0377963267950654 -0.383769047331231
-0.0367963267950655 -0.383365963258221
-0.0357963267950656 -0.382962868911275
-0.0347963267950657 -0.382559763614776
-0.0337963267950658 -0.382156646693043
-0.0327963267950659 -0.381753517470324
-0.0317963267950661 -0.381350375270791
-0.0307963267950662 -0.380947219418538
-0.0297963267950663 -0.380544049237578
-0.0287963267950664 -0.380140864051835
-0.0277963267950665 -0.379737663185145
-0.0267963267950666 -0.379334445961246
-0.0257963267950667 -0.378931211703779
-0.0247963267950668 -0.378527959736282
-0.0237963267950669 -0.378124689382184
-0.022796326795067 -0.377721399964805
-0.0217963267950672 -0.377318090807348
-0.0207963267950673 -0.376914761232898
-0.0197963267950674 -0.376511410564413
-0.0187963267950675 -0.376108038124728
-0.0177963267950676 -0.375704643236543
-0.0167963267950677 -0.375301225222422
-0.0157963267950678 -0.374897783403435
-0.0147963267950679 -0.374494317082285
-0.013796326795068 -0.374090825603589
-0.0127963267950681 -0.373687308289221
-0.0117963267950683 -0.373283764460906
-0.0107963267950684 -0.37288019344022
-0.00979632679506848 -0.372476594548589
-0.00879632679506859 -0.372072967055656
-0.0077963267950687 -0.371669310369985
-0.00679632679506881 -0.371265623798427
-0.00579632679506892 -0.370861906650675
-0.00479632679506903 -0.370458158241033
-0.00379632679506914 -0.370054377886022
-0.00279632679506925 -0.369650564904507
-0.00179632679506936 -0.369246718881917
-0.000796326795069469 -0.368842838352823
0.000203673204930421 -0.368438923560691
0.00120367320493031 -0.368034973265814
0.0022036732049302 -0.367630987009875
0.00320367320493009 -0.36722696371427
0.00420367320492998 -0.366822903269587
0.00520367320492987 -0.366418804764082
0.00620367320492976 -0.366014667516644
0.00720367320492965 -0.365610490850666
0.00820367320492954 -0.365206274093737
0.00920367320492943 -0.364802016579383
0.0102036732049293 -0.364397717493162
0.0112036732049292 -0.363993376235056
0.0122036732049291 -0.363588992127803
0.013203673204929 -0.363184564487945
0.0142036732049289 -0.362780092631767
0.0152036732049288 -0.362375575875289
0.0162036732049287 -0.361971013534262
0.0172036732049285 -0.361566404924162
0.0182036732049284 -0.361161749360187
0.0192036732049283 -0.360757046157251
0.0202036732049282 -0.360352294629977
0.0212036732049281 -0.359947494092697
0.022203673204928 -0.359542643859448
0.0232036732049279 -0.359137743243961
0.0242036732049278 -0.358732791559663
0.0252036732049277 -0.358327788119671
0.0262036732049276 -0.357922732236787
0.0272036732049274 -0.357517623223496
0.0282036732049273 -0.357112460391957
0.0292036732049272 -0.356707243054004
0.0302036732049271 -0.356301970521139
0.031203673204927 -0.355896642104527
0.0322036732049269 -0.355491257114995
0.0332036732049268 -0.355085814863024
0.0342036732049267 -0.354680314658748
0.0352036732049266 -0.354274755811946
0.0362036732049265 -0.353869137632042
0.0372036732049263 -0.353463459428098
0.0382036732049262 -0.35305772050881
0.0392036732049261 -0.352651920182504
0.040203673204926 -0.352246057757134
0.0412036732049259 -0.351840132540272
0.0422036732049258 -0.351434143839111
0.0432036732049257 -0.351028090960454
0.0442036732049256 -0.350621973210714
0.0452036732049255 -0.35021578989591
0.0462036732049254 -0.349809540321658
0.0472036732049252 -0.349403223793171
0.0482036732049251 -0.348996839615256
0.049203673204925 -0.348590387092303
0.0502036732049249 -0.348183865528289
0.0512036732049248 -0.347777274226767
0.0522036732049247 -0.347370612490864
0.0532036732049246 -0.346963879623279
0.0542036732049245 -0.346557074926276
0.0552036732049244 -0.346150197701678
0.0562036732049243 -0.345743247250867
0.0572036732049241 -0.345336222874779
0.058203673204924 -0.344929123873895
0.0592036732049239 -0.344521949548338
0.0602036732049238 -0.344114699197874
0.0612036732049237 -0.3437073721213
0.0622036732049236 -0.343299967617248
0.0632036732049235 -0.342892484983877
0.0642036732049234 -0.342484923518864
0.0652036732049233 -0.342077282519409
0.0662036732049232 -0.341669561282221
0.067203673204923 -0.341261759103521
0.0682036732049229 -0.340853875279032
0.0692036732049228 -0.340445909103978
0.0702036732049227 -0.340037859873079
0.0712036732049226 -0.339629726880544
0.0722036732049225 -0.339221509420072
0.0732036732049224 -0.338813206784841
0.0742036732049223 -0.338404818267509
0.0752036732049222 -0.337996343160208
0.0762036732049221 -0.337587780754535
0.0772036732049219 -0.337179130341557
0.0782036732049218 -0.336770391211796
0.0792036732049217 -0.336361562655232
0.0802036732049216 -0.335952643961297
0.0812036732049215 -0.335543634418867
0.0822036732049214 -0.335134533316263
0.0832036732049213 -0.33472533994124
0.0842036732049212 -0.334316053580989
0.0852036732049211 -0.333906673522129
0.0862036732049209 -0.333497199050702
0.0872036732049208 -0.33308762945217
0.0882036732049207 -0.332677964011412
0.0892036732049206 -0.332268202012714
0.0902036732049205 -0.33185834273977
0.0912036732049204 -0.331448385475675
0.0922036732049203 -0.331038329502921
0.0932036732049202 -0.330628174103392
0.0942036732049201 -0.330217918558359
0.09520367320492 -0.329807562148479
0.0962036732049198 -0.329397104153783
0.0972036732049197 -0.328986543853679
0.0982036732049196 -0.328575880526945
0.0992036732049195 -0.32816511345172
0.100203673204919 -0.327754241905506
0.101203673204919 -0.327343265165161
0.102203673204919 -0.326932182506891
0.103203673204919 -0.326520993206251
0.104203673204919 -0.326109696538136
0.105203673204919 -0.325698291776778
0.106203673204919 -0.32528677819574
0.107203673204919 -0.324875155067915
0.108203673204919 -0.324463421665516
0.109203673204918 -0.324051577260077
0.110203673204918 -0.323639621122443
0.111203673204918 -0.323227552522766
0.112203673204918 -0.322815370730506
0.113203673204918 -0.322403075014417
0.114203673204918 -0.32199066464255
0.115203673204918 -0.321578138882243
0.116203673204918 -0.321165497000118
0.117203673204918 -0.320752738262075
0.118203673204917 -0.320339861933287
0.119203673204917 -0.319926867278192
0.120203673204917 -0.319513753560488
0.121203673204917 -0.319100520043125
0.122203673204917 -0.318687165988293
0.123203673204917 -0.318273690657407
0.124203673204917 -0.3178600933127
0.125203673204917 -0.317446373215208
0.126203673204917 -0.317032529621577
0.127203673204916 -0.316618561790361
0.128203673204916 -0.31620446897931
0.129203673204916 -0.315790250445381
0.130203673204916 -0.315375905444734
0.131203673204916 -0.314961433232736
0.132203673204916 -0.314546833063902
0.133203673204916 -0.314132104191679
0.134203673204916 -0.313717245869427
0.135203673204916 -0.313302257349323
0.136203673204915 -0.312887137882737
0.137203673204915 -0.312471886720225
0.138203673204915 -0.312056503111526
0.139203673204915 -0.311640986305555
0.140203673204915 -0.311225334941181
0.141203673204915 -0.310809549563452
0.142203673204915 -0.310393628544974
0.143203673204915 -0.309977571481633
0.144203673204915 -0.309561377442511
0.145203673204914 -0.309145045655512
0.146203673204914 -0.308728575388655
0.147203673204914 -0.308311965884103
0.148203673204914 -0.307895216383124
0.149203673204914 -0.307478326126085
0.150203673204914 -0.307061294351944
0.151203673204914 -0.306644120294015
0.152203673204914 -0.306226803196628
0.153203673204914 -0.305809342296559
0.154203673204913 -0.305391736829682
0.155203673204913 -0.30497398603097
0.156203673204913 -0.304556089134485
0.157203673204913 -0.304138045373378
0.158203673204913 -0.303719853979878
0.159203673204913 -0.303301514185294
0.160203673204913 -0.302883025220003
0.161203673204913 -0.30246438631345
0.162203673204913 -0.302045596694144
0.163203673204912 -0.30162665558965
0.164203673204912 -0.301207562226587
0.165203673204912 -0.300788315830625
0.166203673204912 -0.300368915626483
0.167203673204912 -0.299949360837925
0.168203673204912 -0.299529650687763
0.169203673204912 -0.299109784539527
0.170203673204912 -0.298689761314301
0.171203673204912 -0.298269580389399
0.172203673204911 -0.297849240983606
0.173203673204911 -0.297428742314708
0.174203673204911 -0.297008083599484
0.175203673204911 -0.296587264053705
0.176203673204911 -0.296166282892124
0.177203673204911 -0.295745139328477
0.178203673204911 -0.295323832575469
0.179203673204911 -0.294902361844777
0.180203673204911 -0.294480726347039
0.18120367320491 -0.294058925291854
0.18220367320491 -0.293636957887769
0.18320367320491 -0.293214823342281
0.18420367320491 -0.292792520861826
0.18520367320491 -0.29237004965178
0.18620367320491 -0.291947408916445
0.18720367320491 -0.291524597859051
0.18820367320491 -0.291101615681747
0.18920367320491 -0.290678461585596
0.190203673204909 -0.290255134770571
0.191203673204909 -0.289831634435546
0.192203673204909 -0.289407959778294
0.193203673204909 -0.288984109995481
0.194203673204909 -0.288560084282658
0.195203673204909 -0.288135881834258
0.196203673204909 -0.28771150184359
0.197203673204909 -0.287286943502831
0.198203673204909 -0.286862206003025
0.199203673204909 -0.286437288534073
0.200203673204908 -0.286012190284729
0.201203673204908 -0.285586910442595
0.202203673204908 -0.285161448194116
0.203203673204908 -0.28473580272457
0.204203673204908 -0.28430997321807
0.205203673204908 -0.28388395885755
0.206203673204908 -0.283457758824764
0.207203673204908 -0.28303137230028
0.208203673204908 -0.282604798463475
0.209203673204907 -0.282178036492525
0.210203673204907 -0.281751085564404
0.211203673204907 -0.281323944854876
0.212203673204907 -0.28089661353849
0.213203673204907 -0.280469090788573
0.214203673204907 -0.280041375777227
0.215203673204907 -0.279613467675318
0.216203673204907 -0.279185365652293
0.217203673204907 -0.27875706887607
0.218203673204906 -0.278328576514455
0.219203673204906 -0.277899887733326
0.220203673204906 -0.277471001697298
0.221203673204906 -0.277041917569718
0.222203673204906 -0.27661263451266
0.223203673204906 -0.276183151686916
0.224203673204906 -0.275753468251993
0.225203673204906 -0.275323583366109
0.226203673204906 -0.274893496186181
0.227203673204905 -0.274463205867821
0.228203673204905 -0.274032711565336
0.229203673204905 -0.273602012431711
0.230203673204905 -0.273171107618615
0.231203673204905 -0.272739996276385
0.232203673204905 -0.272308677554024
0.233203673204905 -0.271877150599197
0.234203673204905 -0.271445414558222
0.235203673204905 -0.271013468576064
0.236203673204904 -0.27058131179633
0.237203673204904 -0.27014894336126
0.238203673204904 -0.269716362411727
0.239203673204904 -0.269283568087223
0.240203673204904 -0.268850559525862
0.241203673204904 -0.268417335864361
0.242203673204904 -0.267983896238049
0.243203673204904 -0.267550239780847
0.244203673204904 -0.26711636562527
0.245203673204903 -0.266682272902421
0.246203673204903 -0.266247960741977
0.247203673204903 -0.265813428272193
0.248203673204903 -0.265378674619885
};
\addplot [semithick, blue]
table {%
0.249203673204903 -0.0687237834648792
0.250203673204903 -0.0680459126919608
0.251203673204903 -0.067367751479357
0.252203673204903 -0.0666892989073478
0.253203673204903 -0.0660105540553301
0.254203673204902 -0.0653315160018148
0.255203673204902 -0.0646521838244247
0.256203673204902 -0.0639725565998924
0.257203673204902 -0.0632926334040579
0.258203673204902 -0.0626124133118661
0.259203673204902 -0.0619318953973648
0.260203673204902 -0.0612510787337028
0.261203673204902 -0.0605699623931265
0.262203673204902 -0.0598885454469789
0.263203673204901 -0.0592068269656963
0.264203673204901 -0.0585248060188072
0.265203673204901 -0.0578424816749289
0.266203673204901 -0.0571598530017659
0.267203673204901 -0.0564769190661074
0.268203673204901 -0.0557936789338254
0.269203673204901 -0.0551101316698719
0.270203673204901 -0.0544262763382774
0.271203673204901 -0.0537421120021481
0.2722036732049 -0.0530576377236636
0.2732036732049 -0.0523728525640756
0.2742036732049 -0.0516877555837042
0.2752036732049 -0.0510023458419372
0.2762036732049 -0.050316622397227
0.2772036732049 -0.0496305843070886
0.2782036732049 -0.0489442306280974
0.2792036732049 -0.0482575604158867
0.2802036732049 -0.0475705727251466
0.281203673204899 -0.0468832666096204
0.282203673204899 -0.0461956411221035
0.283203673204899 -0.0455076953144404
0.284203673204899 -0.0448194282375234
0.285203673204899 -0.0441308389412895
0.286203673204899 -0.0434419264747188
0.287203673204899 -0.0427526898858326
0.288203673204899 -0.0420631282216904
0.289203673204899 -0.0413732405283889
0.290203673204898 -0.0406830258510585
0.291203673204898 -0.0399924832338622
0.292203673204898 -0.0393016117199933
0.293203673204898 -0.0386104103516727
0.294203673204898 -0.0379188781701474
0.295203673204898 -0.0372270142156883
0.296203673204898 -0.0365348175275879
0.297203673204898 -0.035842287144158
0.298203673204898 -0.0351494221027283
0.299203673204897 -0.0344562214396432
0.300203673204897 -0.033762684190261
0.301203673204897 -0.0330688093889507
0.302203673204897 -0.0323745960690909
0.303203673204897 -0.0316800432630666
0.304203673204897 -0.0309851500022682
0.305203673204897 -0.030289915317089
0.306203673204897 -0.0295943382369226
0.307203673204897 -0.028898417790162
0.308203673204896 -0.0282021530041964
0.309203673204896 -0.0275055429054101
0.310203673204896 -0.0268085865191798
0.311203673204896 -0.0261112828698729
0.312203673204896 -0.0254136309808453
0.313203673204896 -0.0247156298744396
0.314203673204896 -0.024017278571983
0.315203673204896 -0.0233185760937849
0.316203673204896 -0.0226195214591355
0.317203673204896 -0.0219201136863037
0.318203673204895 -0.0212203517925349
0.319203673204895 -0.0205202347940487
0.320203673204895 -0.0198197617060379
0.321203673204895 -0.0191189315426657
0.322203673204895 -0.0184177433170637
0.323203673204895 -0.0177161960413307
0.324203673204895 -0.0170142887265301
0.325203673204895 -0.016312020382688
0.326203673204895 -0.0156093900187915
0.327203673204894 -0.0149063966427869
0.328203673204894 -0.0142030392615771
0.329203673204894 -0.0134993168810205
0.330203673204894 -0.0127952285059288
0.331203673204894 -0.0120907731400646
0.332203673204894 -0.0113859497861405
0.333203673204894 -0.0106807574458163
0.334203673204894 -0.00997519511969733
0.335203673204894 -0.00926926180733329
0.336203673204893 -0.00856295650721527
0.337203673204893 -0.00785627821677451
0.338203673204893 -0.00714922593238111
0.339203673204893 -0.00644179864934083
0.340203673204893 -0.00573399536189411
0.341203673204893 -0.00502581506321456
0.342203673204893 -0.00431725674540645
0.343203673204893 -0.00360831939950306
0.344203673204893 -0.00289900201546495
0.345203673204892 -0.00218930358217856
0.346203673204892 -0.00147922308745377
0.347203673204892 -0.000768759518022308
0.348203673204892 -5.79118595364271e-05
0.349203673204892 0.000653320903433348
0.350203673204892 0.00136493978739983
0.351203673204892 0.00207694580996117
0.352203673204892 0.00278933998980192
0.353203673204892 0.00350212334669518
0.354203673204891 0.00421529690150461
0.355203673204891 0.00492886167618554
0.356203673204891 0.00564281869378714
0.357203673204891 0.00635716897845408
0.358203673204891 0.00707191355542748
0.359203673204891 0.00778705345104774
0.360203673204891 0.00850258969275548
0.361203673204891 0.0092185233090934
0.362203673204891 0.00993485532970756
0.36320367320489 0.0106515867853497
0.36420367320489 0.0113687187078782
0.36520367320489 0.0120862521302605
0.36620367320489 0.0128041880865735
0.36720367320489 0.0135225276120064
0.36820367320489 0.0142412717428615
0.36920367320489 0.0149604215165561
0.37020367320489 0.015679977971624
0.37120367320489 0.0163999421477169
0.372203673204889 0.0171203150856065
0.373203673204889 0.0178410978271851
0.374203673204889 0.018562291415468
0.375203673204889 0.0192838968945949
0.376203673204889 0.0200059153098306
0.377203673204889 0.0207283477075674
0.378203673204889 0.0214511951353265
0.379203673204889 0.0221744586417587
0.380203673204889 0.0228981392766471
0.381203673204888 0.0236222380909072
0.382203673204888 0.0243467561365892
0.383203673204888 0.0250716944668796
0.384203673204888 0.0257970541361017
0.385203673204888 0.0265228361997181
0.386203673204888 0.0272490417143313
0.387203673204888 0.027975671737685
0.388203673204888 0.0287027273286664
0.389203673204888 0.0294302095473067
0.390203673204887 0.0301581194547826
0.391203673204887 0.0308864581134182
0.392203673204887 0.0316152265866853
0.393203673204887 0.0323444259392059
0.394203673204887 0.0330740572367526
0.395203673204887 0.03380412154625
0.396203673204887 0.0345346199357766
0.397203673204887 0.0352655534745655
0.398203673204887 0.0359969232330056
0.399203673204886 0.0367287302826433
0.400203673204886 0.0374609756961832
0.401203673204886 0.0381936605474898
0.402203673204886 0.0389267859115884
0.403203673204886 0.0396603528646663
0.404203673204886 0.0403943624840743
0.405203673204886 0.0411288158483273
0.406203673204886 0.0418637140371057
0.407203673204886 0.0425990581312568
0.408203673204885 0.0433348492127958
0.409203673204885 0.0440710883649066
0.410203673204885 0.044807776671943
0.411203673204885 0.0455449152194303
0.412203673204885 0.0462825050940655
0.413203673204885 0.0470205473837191
0.414203673204885 0.0477590431774358
0.415203673204885 0.0484979935654356
0.416203673204885 0.0492373996391145
0.417203673204884 0.0499772624910461
0.418203673204884 0.050717583214982
0.419203673204884 0.0514583629058533
0.420203673204884 0.052199602659771
0.421203673204884 0.0529413035740274
0.422203673204884 0.0536834667470963
0.423203673204884 0.0544260932786355
0.424203673204884 0.0551691842694854
0.425203673204884 0.0559127408216719
0.426203673204884 0.0566567640384062
0.427203673204883 0.0574012550240858
0.428203673204883 0.0581462148842953
0.429203673204883 0.0588916447258077
0.430203673204883 0.0596375456565845
0.431203673204883 0.0603839187857768
0.432203673204883 0.0611307652237262
0.433203673204883 0.0618780860819657
0.434203673204883 0.0626258824732192
0.435203673204883 0.0633741555114043
0.436203673204882 0.0641229063116306
0.437203673204882 0.0648721359902027
0.438203673204882 0.0656218456646193
0.439203673204882 0.0663720364535743
0.440203673204882 0.0671227094769574
0.441203673204882 0.0678738658558552
0.442203673204882 0.0686255067125505
0.443203673204882 0.0693776331705245
0.444203673204882 0.0701302463544563
0.445203673204881 0.0708833473902235
0.446203673204881 0.0716369374049034
0.447203673204881 0.0723910175267725
0.448203673204881 0.0731455888853079
0.449203673204881 0.0739006526111874
0.450203673204881 0.0746562098362893
0.451203673204881 0.0754122616936945
0.452203673204881 0.0761688093176846
0.453203673204881 0.0769258538437451
0.45420367320488 0.0776833964085625
0.45520367320488 0.0784414381500278
0.45620367320488 0.0791999802072346
0.45720367320488 0.0799590237204804
0.45820367320488 0.0807185698312666
0.45920367320488 0.0814786196822994
0.46020367320488 0.0822391744174886
0.46120367320488 0.0830002351819497
0.46220367320488 0.0837618031220023
0.463203673204879 0.0845238793851718
0.464203673204879 0.085286465120189
0.465203673204879 0.0860495614769895
0.466203673204879 0.0868131695489229
0.467203673204879 0.0875772906050128
0.468203673204879 0.088341925739927
0.469203673204879 0.0891070761084243
0.470203673204879 0.0898727428664697
0.471203673204879 0.0906389271712336
0.472203673204878 0.0914056301810932
0.473203673204878 0.0921728530556305
0.474203673204878 0.0929405969556343
0.475203673204878 0.0937088630430986
0.476203673204878 0.0944776524812232
0.477203673204878 0.0952469664344136
0.478203673204878 0.0960168060682807
0.479203673204878 0.0967871725496406
0.480203673204878 0.0975580670465146
0.481203673204877 0.0983294907281288
0.482203673204877 0.0991014447649139
0.483203673204877 0.0998739303285055
0.484203673204877 0.100646948591743
0.485203673204877 0.101420500728669
0.486203673204877 0.10219458791453
0.487203673204877 0.102969211325777
0.488203673204877 0.103744372140062
0.489203673204877 0.10452007153624
0.490203673204876 0.105296310694368
0.491203673204876 0.106073090795705
0.492203673204876 0.10685041302271
0.493203673204876 0.107628278559043
0.494203673204876 0.108406688589565
0.495203673204876 0.109185644300335
0.496203673204876 0.109965146878612
0.497203673204876 0.110745197512852
0.498203673204876 0.111525797392711
0.499203673204875 0.112306947709039
0.500203673204875 0.113088649653885
0.501203673204875 0.113870904420492
0.502203673204875 0.114653713203299
0.503203673204875 0.115437077197938
0.504203673204875 0.116220997601234
0.505203673204875 0.117005475611207
0.506203673204875 0.117790512427067
0.507203673204875 0.118576109249215
0.508203673204874 0.119362267279241
0.509203673204874 0.120148987719926
0.510203673204874 0.120936271775237
0.511203673204874 0.121724120650329
0.512203673204874 0.122512535551545
0.513203673204874 0.123301517686408
0.514203673204874 0.12409106826363
0.515203673204874 0.124881188493104
0.516203673204874 0.125671879585903
0.517203673204873 0.126463142754284
0.518203673204873 0.12725497921168
0.519203673204873 0.128047390172704
0.520203673204873 0.128840376853145
0.521203673204873 0.129633940469969
0.522203673204873 0.130428082241315
0.523203673204873 0.131222803386495
0.524203673204873 0.132018105125993
0.525203673204873 0.132813988681463
0.526203673204872 0.133610455275728
0.527203673204872 0.134407506132778
0.528203673204872 0.135205142477769
0.529203673204872 0.13600336553702
0.530203673204872 0.136802176538015
0.531203673204872 0.137601576709398
0.532203673204872 0.138401567280971
0.533203673204872 0.139202149483697
0.534203673204872 0.140003324549691
0.535203673204871 0.140805093712225
0.536203673204871 0.141607458205724
0.537203673204871 0.142410419265763
0.538203673204871 0.143213978129065
0.539203673204871 0.144018136033501
0.540203673204871 0.144822894218089
0.541203673204871 0.145628253922985
0.542203673204871 0.146434216389493
0.543203673204871 0.147240782860052
0.544203673204871 0.14804795457824
0.54520367320487 0.148855732788768
0.54620367320487 0.149664118737482
0.54720367320487 0.15047311367136
0.54820367320487 0.151282718838506
0.54920367320487 0.152092935488152
0.55020367320487 0.152903764870655
0.55120367320487 0.153715208237492
0.55220367320487 0.154527266841261
0.55320367320487 0.155339941935676
0.554203673204869 0.156153234775569
0.555203673204869 0.156967146616881
0.556203673204869 0.157781678716665
0.557203673204869 0.15859683233308
0.558203673204869 0.159412608725391
0.559203673204869 0.160229009153964
0.560203673204869 0.161046034880266
0.561203673204869 0.161863687166861
0.562203673204869 0.162681967277406
0.563203673204868 0.163500876476651
0.564203673204868 0.164320416030432
0.565203673204868 0.165140587205675
0.566203673204868 0.165961391270386
0.567203673204868 0.166782829493651
0.568203673204868 0.167604903145634
0.569203673204868 0.168427613497574
0.570203673204868 0.16925096182178
0.571203673204868 0.170074949391628
0.572203673204867 0.170899577481562
0.573203673204867 0.171724847367083
0.574203673204867 0.172550760324755
0.575203673204867 0.173377317632195
0.576203673204867 0.174204520568073
0.577203673204867 0.175032370412105
0.578203673204867 0.175860868445056
0.579203673204867 0.176690015948731
0.580203673204867 0.177519814205973
0.581203673204866 0.17835026450066
0.582203673204866 0.179181368117701
0.583203673204866 0.180013126343034
0.584203673204866 0.180845540463619
0.585203673204866 0.181678611767439
0.586203673204866 0.182512341543491
0.587203673204866 0.183346731081786
0.588203673204866 0.184181781673344
0.589203673204866 0.18501749461019
0.590203673204865 0.185853871185349
0.591203673204865 0.186690912692846
0.592203673204865 0.187528620427696
0.593203673204865 0.188366995685905
0.594203673204865 0.189206039764463
0.595203673204865 0.190045753961342
0.596203673204865 0.19088613957549
0.597203673204865 0.191727197906827
0.598203673204865 0.192568930256242
0.599203673204864 0.193411337925587
0.600203673204864 0.194254422217673
0.601203673204864 0.195098184436266
0.602203673204864 0.195942625886083
0.603203673204864 0.196787747872787
0.604203673204864 0.19763355170298
0.605203673204864 0.198480038684203
0.606203673204864 0.199327210124929
0.607203673204864 0.200175067334555
0.608203673204863 0.201023611623402
0.609203673204863 0.201872844302711
0.610203673204863 0.20272276668463
0.611203673204863 0.203573380082219
0.612203673204863 0.204424685809439
0.613203673204863 0.205276685181147
0.614203673204863 0.206129379513095
0.615203673204863 0.206982770121919
0.616203673204863 0.20783685832514
0.617203673204862 0.208691645441154
0.618203673204862 0.209547132789226
0.619203673204862 0.210403321689491
0.620203673204862 0.211260213462942
0.621203673204862 0.212117809431427
0.622203673204862 0.212976110917643
0.623203673204862 0.213835119245131
0.624203673204862 0.21469483573827
0.625203673204862 0.215555261722271
0.626203673204861 0.216416398523172
0.627203673204861 0.217278247467831
0.628203673204861 0.218140809883921
0.629203673204861 0.219004087099923
0.630203673204861 0.219868080445122
0.631203673204861 0.220732791249598
0.632203673204861 0.221598220844222
0.633203673204861 0.22246437056065
0.634203673204861 0.223331241731315
0.63520367320486 0.224198835689422
0.63620367320486 0.225067153768941
0.63720367320486 0.225936197304602
0.63820367320486 0.226805967631885
0.63920367320486 0.227676466087018
0.64020367320486 0.228547694006968
0.64120367320486 0.229419652729432
0.64220367320486 0.230292343592835
0.64320367320486 0.23116576793632
0.644203673204859 0.232039927099742
0.645203673204859 0.232914822423662
0.646203673204859 0.233790455249337
0.647203673204859 0.234666826918717
0.648203673204859 0.235543938774436
0.649203673204859 0.236421792159801
0.650203673204859 0.237300388418793
0.651203673204859 0.238179728896052
0.652203673204859 0.239059814936874
0.653203673204859 0.239940647887202
0.654203673204858 0.240822229093618
0.655203673204858 0.241704559903338
0.656203673204858 0.242587641664199
0.657203673204858 0.243471475724658
0.658203673204858 0.24435606343378
0.659203673204858 0.245241406141229
0.660203673204858 0.246127505197265
0.661203673204858 0.247014361952732
0.662203673204858 0.247901977759049
0.663203673204857 0.248790353968208
0.664203673204857 0.249679491932758
0.665203673204857 0.250569393005802
0.666203673204857 0.251460058540988
0.667203673204857 0.252351489892498
0.668203673204857 0.253243688415042
0.669203673204857 0.254136655463848
0.670203673204857 0.255030392394654
0.671203673204857 0.255924900563699
0.672203673204856 0.256820181327718
0.673203673204856 0.257716236043924
0.674203673204856 0.258613066070008
0.675203673204856 0.259510672764127
0.676203673204856 0.260409057484894
0.677203673204856 0.261308221591369
0.678203673204856 0.26220816644305
0.679203673204856 0.263108893399865
0.680203673204856 0.264010403822163
0.681203673204855 0.264912699070699
0.682203673204855 0.265815780506634
0.683203673204855 0.266719649491515
0.684203673204855 0.267624307387274
0.685203673204855 0.268529755556213
0.686203673204855 0.269435995360996
0.687203673204855 0.27034302816464
0.688203673204855 0.271250855330502
0.689203673204855 0.272159478222273
0.690203673204854 0.273068898203964
0.691203673204854 0.273979116639899
0.692203673204854 0.274890134894702
0.693203673204854 0.275801954333289
0.694203673204854 0.276714576320855
0.695203673204854 0.277628002222865
0.696203673204854 0.278542233405046
0.697203673204854 0.279457271233369
0.698203673204854 0.280373117074047
0.699203673204853 0.281289772293517
0.700203673204853 0.282207238258433
0.701203673204853 0.283125516335654
0.702203673204853 0.284044607892232
0.703203673204853 0.284964514295403
0.704203673204853 0.285885236912573
0.705203673204853 0.286806777111309
0.706203673204853 0.287729136259324
0.707203673204853 0.288652315724472
0.708203673204852 0.28957631687473
0.709203673204852 0.290501141078187
0.710203673204852 0.291426789703037
0.711203673204852 0.292353264117562
0.712203673204852 0.293280565690123
0.713203673204852 0.294208695789145
0.714203673204852 0.29513765578311
0.715203673204852 0.296067447040538
0.716203673204852 0.296998070929982
0.717203673204851 0.297929528820007
0.718203673204851 0.298861822079187
0.719203673204851 0.299794952076085
0.720203673204851 0.300728920179244
0.721203673204851 0.301663727757173
0.722203673204851 0.302599376178334
0.723203673204851 0.303535866811131
0.724203673204851 0.304473201023894
0.725203673204851 0.305411380184867
0.72620367320485 0.306350405662196
0.72720367320485 0.307290278823914
0.72820367320485 0.30823100103793
0.72920367320485 0.309172573672012
0.73020367320485 0.310114998093776
0.73120367320485 0.311058275670671
0.73220367320485 0.312002407769966
0.73320367320485 0.312947395758737
0.73420367320485 0.31389324100385
0.735203673204849 0.314839944871951
0.736203673204849 0.315787508729446
0.737203673204849 0.316735933942495
0.738203673204849 0.317685221876989
0.739203673204849 0.318635373898543
0.740203673204849 0.319586391372475
0.741203673204849 0.320538275663797
0.742203673204849 0.321491028137196
0.743203673204849 0.32244465015702
0.744203673204848 0.323399143087265
0.745203673204848 0.32435450829156
0.746203673204848 0.325310747133148
0.747203673204848 0.326267860974874
0.748203673204848 0.327225851179171
0.749203673204848 0.32818471910804
0.750203673204848 0.329144466123038
0.751203673204848 0.330105093585262
0.752203673204848 0.331066602855332
0.753203673204847 0.332028995293375
0.754203673204847 0.332992272259011
0.755203673204847 0.333956435111334
0.756203673204847 0.3349214852089
0.757203673204847 0.335887423909706
0.758203673204847 0.336854252571178
0.759203673204847 0.337821972550149
0.760203673204847 0.33879058520285
0.761203673204847 0.339760091884886
0.762203673204846 0.340730493951224
0.763203673204846 0.341701792756173
0.764203673204846 0.34267398965337
0.765203673204846 0.34364708599576
0.766203673204846 0.344621083135581
0.767203673204846 0.345595982424345
0.768203673204846 0.346571785212822
0.769203673204846 0.34754849285102
0.770203673204846 0.348526106688172
0.771203673204846 0.349504628072713
0.772203673204845 0.350484058352266
0.773203673204845 0.351464398873621
0.774203673204845 0.352445650982718
0.775203673204845 0.353427816024633
0.776203673204845 0.354410895343551
0.777203673204845 0.355394890282755
0.778203673204845 0.356379802184604
0.779203673204845 0.357365632390517
0.780203673204845 0.35835238224095
0.781203673204844 0.359340053075381
0.782203673204844 0.36032864623229
0.783203673204844 0.361318163049138
0.784203673204844 0.362308604862352
0.785203673204844 0.363299973007298
0.786203673204844 0.364292268818273
0.787203673204844 0.365285493628474
0.788203673204844 0.366279648769986
0.789203673204844 0.367274735573758
0.790203673204843 0.368270755369585
0.791203673204843 0.369267709486089
0.792203673204843 0.370265599250695
0.793203673204843 0.371264425989616
0.794203673204843 0.372264191027828
0.795203673204843 0.37326489568905
0.796203673204843 0.37426654129573
0.797203673204843 0.375269129169013
0.798203673204843 0.37627266062873
0.799203673204842 0.377277136993372
0.800203673204842 0.37828255958007
0.801203673204842 0.379288929704576
0.802203673204842 0.380296248681236
0.803203673204842 0.381304517822975
0.804203673204842 0.382313738441273
0.805203673204842 0.383323911846142
0.806203673204842 0.384335039346104
0.807203673204842 0.385347122248174
0.808203673204841 0.386360161857829
0.809203673204841 0.387374159478997
0.810203673204841 0.388389116414024
0.811203673204841 0.38940503396366
0.812203673204841 0.39042191342703
0.813203673204841 0.391439756101617
0.814203673204841 0.392458563283235
0.815203673204841 0.393478336266007
0.816203673204841 0.394499076342345
0.81720367320484 0.395520784802921
0.81820367320484 0.396543462936652
0.81920367320484 0.397567112030667
0.82020367320484 0.398591733370291
0.82120367320484 0.399617328239018
0.82220367320484 0.400643897918489
0.82320367320484 0.401671443688465
0.82420367320484 0.402699966826807
0.82520367320484 0.403729468609448
0.826203673204839 0.404759950310373
0.827203673204839 0.405791413201591
0.828203673204839 0.406823858553111
0.829203673204839 0.407857287632919
0.830203673204839 0.408891701706952
0.831203673204839 0.409927102039074
0.832203673204839 0.41096348989105
0.833203673204839 0.412000866522521
0.834203673204839 0.41303923319098
0.835203673204838 0.414078591151743
0.836203673204838 0.41511894165793
0.837203673204838 0.416160285960432
0.838203673204838 0.417202625307891
0.839203673204838 0.418245960946669
0.840203673204838 0.419290294120827
0.841203673204838 0.420335626072095
0.842203673204838 0.421381958039848
0.843203673204838 0.422429291261078
0.844203673204837 0.42347762697037
0.845203673204837 0.424526966399869
0.846203673204837 0.425577310779263
0.847203673204837 0.426628661335747
0.848203673204837 0.427681019294
0.849203673204837 0.42873438587616
0.850203673204837 0.42978876230179
0.851203673204837 0.430844149787857
0.852203673204837 0.431900549548701
0.853203673204836 0.432957962796009
0.854203673204836 0.434016390738785
0.855203673204836 0.435075834583324
0.856203673204836 0.436136295533184
0.857203673204836 0.437197774789154
0.858203673204836 0.438260273549232
0.859203673204836 0.439323793008591
0.860203673204836 0.440388334359551
0.861203673204836 0.441453898791554
0.862203673204835 0.442520487491131
0.863203673204835 0.443588101641875
0.864203673204835 0.444656742424411
0.865203673204835 0.445726411016366
0.866203673204835 0.446797108592343
0.867203673204835 0.447868836323886
0.868203673204835 0.448941595379455
0.869203673204835 0.450015386924394
0.870203673204835 0.4510902121209
0.871203673204834 0.452166072127996
0.872203673204834 0.453242968101498
0.873203673204834 0.454320901193984
0.874203673204834 0.455399872554769
0.875203673204834 0.456479883329866
0.876203673204834 0.457560934661962
0.877203673204834 0.458643027690383
0.878203673204834 0.459726163551068
0.879203673204834 0.460810343376529
0.880203673204834 0.461895568295831
0.881203673204833 0.462981839434549
0.882203673204833 0.464069157914746
0.883203673204833 0.465157524854935
0.884203673204833 0.466246941370051
0.885203673204833 0.467337408571417
0.886203673204833 0.468428927566711
0.887203673204833 0.469521499459938
0.888203673204833 0.47061512535139
0.889203673204833 0.471709806337624
0.890203673204832 0.472805543511419
0.891203673204832 0.473902337961749
0.892203673204832 0.47500019077375
0.893203673204832 0.476099103028685
0.894203673204832 0.47719907580391
0.895203673204832 0.478300110172844
0.896203673204832 0.479402207204935
0.897203673204832 0.480505367965623
0.898203673204832 0.48160959351631
0.899203673204831 0.482714884914322
0.900203673204831 0.483821243212883
0.901203673204831 0.48492866946107
0.902203673204831 0.486037164703787
0.903203673204831 0.487146729981729
0.904203673204831 0.488257366331345
0.905203673204831 0.489369074784805
0.906203673204831 0.490481856369966
0.907203673204831 0.491595712110336
0.90820367320483 0.492710643025039
0.90920367320483 0.493826650128779
0.91020367320483 0.494943734431808
0.91120367320483 0.496061896939888
0.91220367320483 0.497181138654254
0.91320367320483 0.498301460571583
0.91420367320483 0.499422863683953
0.91520367320483 0.50054534897881
0.91620367320483 0.501668917438934
0.917203673204829 0.502793570042396
0.918203673204829 0.50391930776253
0.919203673204829 0.50504613156789
0.920203673204829 0.506174042422217
0.921203673204829 0.507303041284402
0.922203673204829 0.508433129108446
0.923203673204829 0.509564306843429
0.924203673204829 0.510696575433467
0.925203673204829 0.511829935817678
0.926203673204828 0.512964388930145
0.927203673204828 0.514099935699875
0.928203673204828 0.515236577050768
0.929203673204828 0.516374313901572
0.930203673204828 0.51751314716585
0.931203673204828 0.51865307775194
0.932203673204828 0.519794106562917
0.933203673204828 0.520936234496559
0.934203673204828 0.522079462445299
0.935203673204827 0.523223791296198
0.936203673204827 0.524369221930899
0.937203673204827 0.52551575522559
0.938203673204827 0.526663392050967
0.939203673204827 0.527812133272193
0.940203673204827 0.528961979748861
0.941203673204827 0.530112932334951
0.942203673204827 0.531264991878796
0.943203673204827 0.53241815922304
0.944203673204826 0.533572435204596
0.945203673204826 0.534727820654613
0.946203673204826 0.535884316398429
0.947203673204826 0.537041923255536
0.948203673204826 0.538200642039537
0.949203673204826 0.53936047355811
0.950203673204826 0.540521418612964
0.951203673204826 0.5416834779998
0.952203673204826 0.54284665250827
0.953203673204825 0.544010942921937
0.954203673204825 0.545176350018237
0.955203673204825 0.546342874568433
0.956203673204825 0.547510517337579
0.957203673204825 0.548679279084476
0.958203673204825 0.549849160561632
0.959203673204825 0.551020162515222
0.960203673204825 0.552192285685043
0.961203673204825 0.553365530804477
0.962203673204824 0.55453989860045
0.963203673204824 0.555715389793384
0.964203673204824 0.556892005097163
0.965203673204824 0.558069745219084
0.966203673204824 0.559248610859824
0.967203673204824 0.560428602713389
0.968203673204824 0.561609721467077
0.969203673204824 0.562791967801435
0.970203673204824 0.563975342390215
0.971203673204823 0.565159845900336
0.972203673204823 0.566345478991837
0.973203673204823 0.567532242317834
0.974203673204823 0.568720136524482
0.975203673204823 0.56990916225093
0.976203673204823 0.571099320129277
0.977203673204823 0.572290610784527
0.978203673204823 0.573483034834555
0.979203673204823 0.574676592890052
0.980203673204822 0.57587128555449
0.981203673204822 0.577067113424078
0.982203673204822 0.578264077087712
0.983203673204822 0.579462177126943
0.984203673204822 0.580661414115921
0.985203673204822 0.581861788621362
0.986203673204822 0.583063301202495
0.987203673204822 0.584265952411027
0.988203673204822 0.585469742791093
0.989203673204821 0.586674672879214
0.990203673204821 0.587880743204254
0.991203673204821 0.589087954287373
0.992203673204821 0.590296306641986
0.993203673204821 0.591505800773719
0.994203673204821 0.59271643718036
0.995203673204821 0.59392821635182
0.996203673204821 0.595141138770086
0.997203673204821 0.596355204909176
0.998203673204821 0.597570415235097
0.99920367320482 0.598786770205795
1.00020367320482 0.600004270271119
1.00120367320482 0.601222915872765
1.00220367320482 0.602442707444243
1.00320367320482 0.603663645410823
1.00420367320482 0.604885730189493
1.00520367320482 0.606108962188916
1.00620367320482 0.607333341809381
1.00720367320482 0.608558869442762
1.00820367320482 0.60978554547247
1.00920367320482 0.611013370273409
1.01020367320482 0.61224234421193
1.01120367320482 0.613472467645784
1.01220367320482 0.614703740924082
1.01320367320482 0.615936164387243
1.01420367320482 0.617169738366953
1.01520367320482 0.618404463186118
1.01620367320482 0.619640339158818
1.01720367320482 0.620877366590261
1.01820367320482 0.62211554577674
1.01920367320482 0.623354877005583
1.02020367320482 0.624595360555112
1.02120367320482 0.625836996694592
1.02220367320482 0.627079785684192
1.02320367320482 0.628323727774931
1.02420367320482 0.62956882320864
1.02520367320482 0.630815072217909
1.02620367320482 0.632062475026047
1.02720367320482 0.633311031847032
1.02820367320482 0.634560742885468
1.02920367320482 0.635811608336537
1.03020367320482 0.637063628385953
1.03120367320482 0.638316803209916
1.03220367320482 0.639571132975068
1.03320367320482 0.640826617838446
1.03420367320482 0.642083257947431
1.03520367320482 0.643341053439712
1.03620367320482 0.64460000444323
1.03720367320482 0.645860111076137
1.03820367320482 0.64712137344675
1.03920367320482 0.648383791653502
1.04020367320482 0.649647365784899
1.04120367320482 0.650912095919472
1.04220367320482 0.652177982125731
1.04320367320482 0.65344502446212
1.04420367320482 0.65471322297697
1.04520367320482 0.655982577708453
1.04620367320482 0.657253088684536
1.04720367320482 0.658524755922935
1.04820367320482 0.659797579431069
1.04920367320481 0.661071559206012
1.05020367320481 0.662346695234451
1.05120367320481 0.663622987492638
1.05220367320481 0.664900435946343
1.05320367320481 0.666179040550807
1.05420367320481 0.6674588012507
1.05520367320481 0.668739717980073
1.05620367320481 0.670021790662311
1.05720367320481 0.67130501921009
1.05820367320481 0.672589403525326
1.05920367320481 0.673874943499137
1.06020367320481 0.67516163901179
1.06120367320481 0.676449489932658
1.06220367320481 0.677738496120177
1.06320367320481 0.679028657421796
1.06420367320481 0.680319973673934
1.06520367320481 0.681612444701934
1.06620367320481 0.682906070320018
1.06720367320481 0.684200850331239
1.06820367320481 0.685496784527441
1.06920367320481 0.686793872689207
1.07020367320481 0.68809211458582
1.07120367320481 0.689391509975214
1.07220367320481 0.69069205860393
1.07320367320481 0.691993760207071
1.07420367320481 0.693296614508257
1.07520367320481 0.694600621219581
1.07620367320481 0.695905780041561
1.07720367320481 0.697212090663102
1.07820367320481 0.698519552761442
1.07920367320481 0.699828166002117
1.08020367320481 0.701137930038909
1.08120367320481 0.702448844513807
1.08220367320481 0.703760909056958
1.08320367320481 0.705074123286626
1.08420367320481 0.70638848680915
1.08520367320481 0.707703999218892
1.08620367320481 0.709020660098203
1.08720367320481 0.710338469017372
1.08820367320481 0.711657425534584
1.08920367320481 0.71297752919588
1.09020367320481 0.71429877953511
1.09120367320481 0.715621176073889
1.09220367320481 0.716944718321556
1.09320367320481 0.718269405775131
1.09420367320481 0.719595237919269
1.09520367320481 0.720922214226223
1.09620367320481 0.722250334155794
1.09720367320481 0.723579597155293
1.09820367320481 0.7249100026595
1.09920367320481 0.726241550090615
1.10020367320481 0.727574238858225
1.10120367320481 0.728908068359252
1.10220367320481 0.730243037977919
1.10320367320481 0.731579147085706
1.10420367320481 0.732916395041307
1.10520367320481 0.734254781190588
1.10620367320481 0.735594304866549
1.10720367320481 0.73693496538928
1.10820367320481 0.738276762065922
1.10920367320481 0.739619694190623
1.11020367320481 0.740963761044503
1.11120367320481 0.742308961895607
1.11220367320481 0.743655295998871
1.11320367320481 0.745002762596075
1.11420367320481 0.746351360915809
1.11520367320481 0.747701090173432
1.11620367320481 0.74905194957103
1.11720367320481 0.750403938297379
1.11820367320481 0.751757055527904
1.11920367320481 0.753111300424642
1.12020367320481 0.754466672136202
1.12120367320481 0.755823169797726
1.12220367320481 0.757180792530853
1.12320367320481 0.758539539443677
1.12420367320481 0.759899409630713
1.12520367320481 0.761260402172856
1.12620367320481 0.762622516137346
1.12720367320481 0.763985750577728
1.12820367320481 0.765350104533819
1.12920367320481 0.766715577031665
1.13020367320481 0.768082167083512
1.13120367320481 0.769449873687761
1.13220367320481 0.770818695828941
1.13320367320481 0.772188632477667
1.13420367320481 0.773559682590602
1.13520367320481 0.774931845110431
1.13620367320481 0.776305118965816
1.13720367320481 0.777679503071368
1.13820367320481 0.779054996327605
1.1392036732048 0.780431597620928
1.1402036732048 0.781809305823576
1.1412036732048 0.783188119793599
1.1422036732048 0.784568038374822
1.1432036732048 0.78594906039681
1.1442036732048 0.787331184674839
1.1452036732048 0.788714410009861
1.1462036732048 0.790098735188468
1.1472036732048 0.791484158982867
1.1482036732048 0.792870680150842
1.1492036732048 0.794258297435723
1.1502036732048 0.795647009566359
1.1512036732048 0.797036815257081
1.1522036732048 0.798427713207674
1.1532036732048 0.799819702103349
1.1542036732048 0.801212780614707
1.1552036732048 0.802606947397714
1.1562036732048 0.80400220109367
1.1572036732048 0.805398540329176
1.1582036732048 0.806795963716112
1.1592036732048 0.808194469851604
1.1602036732048 0.809594057317994
1.1612036732048 0.810994724682818
1.1622036732048 0.81239647049877
1.1632036732048 0.813799293303684
1.1642036732048 0.8152031916205
1.1652036732048 0.816608163957238
1.1662036732048 0.818014208806976
1.1672036732048 0.819421324647821
1.1682036732048 0.820829509942881
1.1692036732048 0.822238763140246
1.1702036732048 0.823649082672956
1.1712036732048 0.825060466958983
1.1722036732048 0.826472914401201
1.1732036732048 0.827886423387366
1.1742036732048 0.829300992290091
1.1752036732048 0.830716619466824
1.1762036732048 0.832133303259823
1.1772036732048 0.833551041996137
1.1782036732048 0.83496983398758
1.1792036732048 0.836389677530713
1.1802036732048 0.837810570906821
1.1812036732048 0.839232512381892
1.1822036732048 0.840655500206599
1.1832036732048 0.842079532616275
1.1842036732048 0.843504607830899
1.1852036732048 0.844930724055073
1.1862036732048 0.846357879478004
1.1872036732048 0.847786072273488
1.1882036732048 0.849215300599888
1.1892036732048 0.850645562600119
1.1902036732048 0.85207685640163
1.1912036732048 0.853509180116389
1.1922036732048 0.854942531840864
1.1932036732048 0.856376909656007
1.1942036732048 0.857812311627243
1.1952036732048 0.859248735804448
1.1962036732048 0.860686180221942
1.1972036732048 0.862124642898468
1.1982036732048 0.863564121837184
1.1992036732048 0.865004615025644
1.2002036732048 0.866446120435792
1.2012036732048 0.867888636023942
1.2022036732048 0.869332159730774
1.2032036732048 0.870776689481314
1.2042036732048 0.872222223184932
1.2052036732048 0.873668758735324
1.2062036732048 0.875116294010507
1.2072036732048 0.876564826872805
1.2082036732048 0.878014355168845
1.2092036732048 0.879464876729543
1.2102036732048 0.880916389370101
1.2112036732048 0.882368890889994
1.2122036732048 0.883822379072968
1.2132036732048 0.88527685168703
1.2142036732048 0.88673230648444
1.2152036732048 0.888188741201713
1.2162036732048 0.889646153559604
1.2172036732048 0.89110454126311
1.2182036732048 0.892563902001463
1.2192036732048 0.894024233448127
1.2202036732048 0.895485533260794
1.2212036732048 0.896947799081384
1.2222036732048 0.898411028536037
1.2232036732048 0.899875219235119
1.2242036732048 0.901340368773213
1.2252036732048 0.902806474729124
1.2262036732048 0.904273534665877
1.2272036732048 0.905741546130716
1.2282036732048 0.907210506655109
1.2292036732048 0.908680413754742
1.23020367320479 0.910151264929528
1.23120367320479 0.91162305766361
1.23220367320479 0.913095789425354
1.23320367320479 0.914569457667367
1.23420367320479 0.916044059826487
1.23520367320479 0.9175195933238
1.23620367320479 0.918996055564634
1.23720367320479 0.920473443938576
1.23820367320479 0.921951755819467
1.23920367320479 0.923430988565418
1.24020367320479 0.924911139518813
1.24120367320479 0.926392206006315
1.24220367320479 0.92787418533888
1.24320367320479 0.929357074811762
1.24420367320479 0.930840871704525
1.24520367320479 0.932325573281049
1.24620367320479 0.933811176789547
1.24720367320479 0.935297679462571
1.24820367320479 0.936785078517026
1.24920367320479 0.938273371154184
1.25020367320479 0.939762554559692
1.25120367320479 0.941252625903593
1.25220367320479 0.942743582340332
1.25320367320479 0.94423542100878
1.25420367320479 0.945728139032238
1.25520367320479 0.947221733518465
1.25620367320479 0.948716201559686
1.25720367320479 0.95021154023261
1.25820367320479 0.951707746598453
1.25920367320479 0.953204817702951
1.26020367320479 0.95470275057638
1.26120367320479 0.956201542233577
1.26220367320479 0.95770118967396
1.26320367320479 0.959201689881545
1.26420367320479 0.960703039824972
1.26520367320479 0.962205236457525
1.26620367320479 0.963708276717154
1.26720367320479 0.965212157526497
1.26820367320479 0.966716875792907
1.26920367320479 0.968222428408473
1.27020367320479 0.969728812250046
1.27120367320479 0.971236024179264
1.27220367320479 0.972744061042582
1.27320367320479 0.97425291967129
1.27420367320479 0.97576259688155
1.27520367320479 0.977273089474417
1.27620367320479 0.97878439423587
1.27720367320479 0.980296507936844
1.27820367320479 0.981809427333252
1.27920367320479 0.983323149166024
1.28020367320479 0.984837670161133
1.28120367320479 0.986352987029626
1.28220367320479 0.987869096467661
1.28320367320479 0.989385995156535
1.28420367320479 0.990903679762718
1.28520367320479 0.992422146937891
1.28620367320479 0.993941393318975
1.28720367320479 0.99546141552817
1.28820367320479 0.996982210172991
1.28920367320479 0.998503773846303
1.29020367320479 1.00002610312636
1.29120367320479 1.00154919457683
1.29220367320479 1.00307304474687
1.29320367320479 1.00459765017112
1.29420367320479 1.00612300736976
1.29520367320479 1.00764911284857
1.29620367320479 1.00917596309893
1.29720367320479 1.01070355459791
1.29820367320479 1.01223188380827
1.29920367320479 1.01376094717853
1.30020367320479 1.015290741143
1.30120367320479 1.01682126212182
1.30220367320479 1.01835250652102
1.30320367320479 1.01988447073256
1.30420367320479 1.02141715113436
1.30520367320479 1.02295054409038
1.30620367320479 1.02448464595062
1.30720367320479 1.02601945305122
1.30820367320479 1.02755496171447
1.30920367320479 1.02909116824887
1.31020367320479 1.03062806894918
1.31120367320479 1.03216566009649
1.31220367320479 1.03370393795822
1.31320367320479 1.03524289878823
1.31420367320479 1.03678253882683
1.31520367320479 1.03832285430086
1.31620367320479 1.03986384142374
1.31720367320479 1.04140549639548
1.31820367320479 1.0429478154028
1.31920367320479 1.04449079461915
1.32020367320479 1.04603443020476
1.32120367320478 1.04757871830672
1.32220367320478 1.04912365505903
1.32320367320478 1.05066923658262
1.32420367320478 1.05221545898548
1.32520367320478 1.05376231836264
1.32620367320478 1.0553098107963
1.32720367320478 1.05685793235584
1.32820367320478 1.0584066790979
1.32920367320478 1.05995604706646
1.33020367320478 1.06150603229284
1.33120367320478 1.06305663079584
1.33220367320478 1.06460783858176
1.33320367320478 1.06615965164446
1.33420367320478 1.06771206596544
1.33520367320478 1.06926507751389
1.33620367320478 1.07081868224679
1.33720367320478 1.07237287611397
1.33820367320478 1.07392765503801
1.33920367320478 1.07548301494462
1.34020367320478 1.07703895174249
1.34120367320478 1.0785954613284
1.34220367320478 1.08015253958731
1.34320367320478 1.08171018239241
1.34420367320478 1.08326838560521
1.34520367320478 1.08482714507558
1.34620367320478 1.08638645664186
1.34720367320478 1.08794631613089
1.34820367320478 1.08950671935813
1.34920367320478 1.09106766212768
1.35020367320478 1.0926291402324
1.35120367320478 1.09419114945395
1.35220367320478 1.09575368556289
1.35320367320478 1.09731674431874
1.35420367320478 1.09888032147004
1.35520367320478 1.10044441275448
1.35620367320478 1.10200901389891
1.35720367320478 1.10357412061946
1.35820367320478 1.10513972862162
1.35920367320478 1.10670583360029
1.36020367320478 1.10827243123987
1.36120367320478 1.10983951721436
1.36220367320478 1.1114070871874
1.36320367320478 1.11297513681239
1.36420367320478 1.11454366173255
1.36520367320478 1.116112657581
1.36620367320478 1.11768211998086
1.36720367320478 1.11925204454531
1.36820367320478 1.12082242687768
1.36920367320478 1.12239326257154
1.37020367320478 1.12396454721079
1.37120367320478 1.12553627636971
1.37220367320478 1.12710844561309
1.37320367320478 1.12868105049629
1.37420367320478 1.13025408656532
1.37520367320478 1.13182754935697
1.37620367320478 1.13340143439881
1.37720367320478 1.13497573720938
1.37820367320478 1.13655045329821
1.37920367320478 1.13812557816592
1.38020367320478 1.13970110730432
1.38120367320478 1.14127703619651
1.38220367320478 1.14285336031693
1.38320367320478 1.14443007513149
1.38420367320478 1.14600717609765
1.38520367320478 1.14758465866448
1.38620367320478 1.14916251827282
1.38720367320478 1.15074075035528
1.38820367320478 1.15231935033643
1.38920367320478 1.1538983136328
1.39020367320478 1.15547763565305
1.39120367320478 1.15705731179801
1.39220367320478 1.15863733746082
1.39320367320478 1.16021770802696
1.39420367320478 1.16179841887443
1.39520367320478 1.16337946537376
1.39620367320478 1.16496084288816
1.39720367320478 1.1665425467736
1.39820367320478 1.16812457237891
1.39920367320478 1.16970691504587
1.40020367320478 1.17128957010931
1.40120367320478 1.17287253289721
1.40220367320478 1.17445579873079
1.40320367320478 1.17603936292461
1.40420367320478 1.17762322078669
1.40520367320478 1.17920736761858
1.40620367320478 1.18079179871546
1.40720367320478 1.18237650936627
1.40820367320478 1.18396149485377
1.40920367320478 1.18554675045467
1.41020367320478 1.18713227143973
1.41120367320478 1.18871805307383
1.41220367320477 1.19030409061611
1.41320367320477 1.19189037932004
1.41420367320477 1.19347691443354
1.41520367320477 1.19506369119908
1.41620367320477 1.19665070485378
1.41720367320477 1.19823795062952
1.41820367320477 1.19982542375301
1.41920367320477 1.20141311944594
1.42020367320477 1.20300103292506
1.42120367320477 1.20458915940229
1.42220367320477 1.2061774940848
1.42320367320477 1.20776603217516
1.42420367320477 1.20935476887139
1.42520367320477 1.21094369936712
1.42620367320477 1.21253281885166
1.42720367320477 1.2141221225101
1.42820367320477 1.21571160552345
1.42920367320477 1.2173012630687
1.43020367320477 1.21889109031898
1.43120367320477 1.22048108244362
1.43220367320477 1.22207123460827
1.43320367320477 1.22366154197502
1.43420367320477 1.22525199970249
1.43520367320477 1.22684260294593
1.43620367320477 1.22843334685738
1.43720367320477 1.23002422658569
1.43820367320477 1.23161523727671
1.43920367320477 1.23320637407335
1.44020367320477 1.23479763211569
1.44120367320477 1.23638900654112
1.44220367320477 1.23798049248441
1.44320367320477 1.23957208507783
1.44420367320477 1.24116377945129
1.44520367320477 1.24275557073239
1.44620367320477 1.24434745404658
1.44720367320477 1.24593942451725
1.44820367320477 1.24753147726581
1.44920367320477 1.24912360741186
1.45020367320477 1.25071581007325
1.45120367320477 1.2523080803662
1.45220367320477 1.25390041340543
1.45320367320477 1.25549280430425
1.45420367320477 1.25708524817465
1.45520367320477 1.25867774012745
1.45620367320477 1.2602702752724
1.45720367320477 1.26186284871827
1.45820367320477 1.26345545557296
1.45920367320477 1.26504809094365
1.46020367320477 1.26664074993685
1.46120367320477 1.26823342765855
1.46220367320477 1.26982611921434
1.46320367320477 1.27141881970946
1.46420367320477 1.27301152424899
1.46520367320477 1.27460422793789
1.46620367320477 1.27619692588115
1.46720367320477 1.2777896131839
1.46820367320477 1.27938228495148
1.46920367320477 1.28097493628961
1.47020367320477 1.28256756230444
1.47120367320477 1.28416015810272
1.47220367320477 1.28575271879185
1.47320367320477 1.28734523929471
1.47420367320477 1.28893771509445
1.47520367320477 1.29053014111252
1.47620367320477 1.29212251246013
1.47720367320477 1.29371482424971
1.47820367320477 1.29530707159506
1.47920367320477 1.29689924961141
1.48020367320477 1.29849135341553
1.48120367320477 1.30008337812589
1.48220367320477 1.30167531886031
1.48320367320477 1.30326717073064
1.48420367320477 1.30485892887443
1.48520367320477 1.30645058841784
1.48620367320477 1.30804214448921
1.48720367320477 1.30963359221923
1.48820367320477 1.31122492674098
1.48920367320477 1.3128161431901
1.49020367320477 1.31440723670489
1.49120367320477 1.31599820242637
1.49220367320477 1.31758903549846
1.49320367320477 1.31917973106802
1.49420367320477 1.32077028428502
1.49520367320477 1.32236069030262
1.49620367320477 1.32395094427727
1.49720367320477 1.32554104136884
1.49820367320477 1.3271309767407
1.49920367320477 1.32872074555989
1.50020367320477 1.33031034299714
1.50120367320477 1.33189976422708
1.50220367320476 1.33348900442826
1.50320367320476 1.33507805878332
1.50420367320476 1.33666692247908
1.50520367320476 1.33825559070664
1.50620367320476 1.3398440586607
1.50720367320476 1.3414323215268
1.50820367320476 1.34302037452136
1.50920367320476 1.3446082128532
1.51020367320476 1.34619583173591
1.51120367320476 1.34778322638793
1.51220367320476 1.34937039203269
1.51320367320476 1.3509573238987
1.51420367320476 1.35254401721962
1.51520367320476 1.35413046723443
1.51620367320476 1.35571666918749
1.51720367320476 1.35730261832863
1.51820367320476 1.35888830991328
1.51920367320476 1.36047373920256
1.52020367320476 1.36205890146339
1.52120367320476 1.36364379196858
1.52220367320476 1.36522840599692
1.52320367320476 1.36681273883332
1.52420367320476 1.36839678576888
1.52520367320476 1.36998054210097
1.52620367320476 1.37156400313339
1.52720367320476 1.37314716417641
1.52820367320476 1.37473002054689
1.52920367320476 1.3763125675684
1.53020367320476 1.37789480057129
1.53120367320476 1.37947671489278
1.53220367320476 1.38105830587711
1.53320367320476 1.38263956887555
1.53420367320476 1.3842204992466
1.53520367320476 1.38580109235599
1.53620367320476 1.38738134357685
1.53720367320476 1.38896124828975
1.53820367320476 1.39054080188284
1.53920367320476 1.39211999975191
1.54020367320476 1.39369883730049
1.54120367320476 1.39527730993998
1.54220367320476 1.3968554130897
1.54320367320476 1.39843314217698
1.54420367320476 1.4000104926373
1.54520367320476 1.40158745991435
1.54620367320476 1.40316403946009
1.54720367320476 1.40474022673492
1.54820367320476 1.4063160172077
1.54920367320476 1.40789140635587
1.55020367320476 1.40946638966555
1.55120367320476 1.41104096263161
1.55220367320476 1.41261512075775
1.55320367320476 1.41418885955662
1.55420367320476 1.41576217454989
1.55520367320476 1.41733506126834
1.55620367320476 1.41890751525195
1.55720367320476 1.42047953204997
1.55820367320476 1.42205110722104
1.55920367320476 1.42362223633325
1.56020367320476 1.42519291496422
1.56120367320476 1.42676313870121
1.56220367320476 1.4283329031412
1.56320367320476 1.42990220389097
1.56420367320476 1.43147103656717
1.56520367320476 1.43303939679644
1.56620367320476 1.43460728021978
1.56720367320476 1.43617468248778
1.56820367320476 1.43774159924958
1.56920367320476 1.43930802597588
};
\addplot [semithick, red, dashed]
table {%
-1.5707963267949 -1.5707963267949
1.57020367320476 1.57020367320476
};
\addplot [semithick, green!50!black]
table {%
0 0
0 -0.368521192865343
-0.368521192865343 -0.368521192865343
-0.368521192865343 -0.721467587207198
-0.721467587207198 -0.721467587207198
-0.721467587207198 -0.617047812550744
-0.617047812550744 -0.617047812550744
-0.617047812550744 -0.579945407941976
-0.579945407941976 -0.579945407941976
-0.579945407941976 -0.577666048319931
-0.577666048319931 -0.577666048319931
-0.577666048319931 -0.584062548461944
-0.584062548461944 -0.584062548461944
-0.584062548461944 -0.565937826043022
-0.565937826043022 -0.565937826043022
-0.565937826043022 -0.615914054085813
-0.615914054085813 -0.615914054085813
-0.615914054085813 -0.581348915281857
-0.581348915281857 -0.581348915281857
-0.581348915281857 -0.573693318981791
-0.573693318981791 -0.573693318981791
-0.573693318981791 -0.59504891913752
-0.59504891913752 -0.59504891913752
-0.59504891913752 -0.577697046608726
-0.577697046608726 -0.577697046608726
-0.577697046608726 -0.583976016484325
-0.583976016484325 -0.583976016484325
-0.583976016484325 -0.566186653218266
-0.566186653218266 -0.566186653218266
-0.566186653218266 -0.61525637572078
-0.61525637572078 -0.61525637572078
-0.61525637572078 -0.536577339200728
-0.536577339200728 -0.536577339200728
-0.536577339200728 -0.692047213134898
-0.692047213134898 -0.692047213134898
-0.692047213134898 -0.561844090574093
-0.561844090574093 -0.561844090574093
-0.561844090574093 -0.626624321163496
-0.626624321163496 -0.626624321163496
-0.626624321163496 -0.567877324874506
-0.567877324874506 -0.567877324874506
-0.567877324874506 -0.610767275120329
-0.610767275120329 -0.610767275120329
-0.610767275120329 -0.545998065518524
-0.545998065518524 -0.545998065518524
-0.545998065518524 -0.660814103455166
-0.660814103455166 -0.660814103455166
-0.660814103455166 -0.583410908559691
-0.583410908559691 -0.583410908559691
-0.583410908559691 -0.567809179708106
-0.567809179708106 -0.567809179708106
-0.567809179708106 -0.610948907319307
-0.610948907319307 -0.610948907319307
-0.610948907319307 -0.545620139393814
-0.545620139393814 -0.545620139393814
-0.545620139393814 -0.662099998963579
-0.662099998963579 -0.662099998963579
-0.662099998963579 -0.582561090946836
-0.582561090946836 -0.582561090946836
-0.582561090946836 -0.570241107622274
-0.570241107622274 -0.570241107622274
-0.570241107622274 -0.604430720994543
-0.604430720994543 -0.604430720994543
-0.604430720994543 -0.559014075187678
-0.559014075187678 -0.559014075187678
-0.559014075187678 -0.633908520194949
-0.633908520194949 -0.633908520194949
-0.633908520194949 -0.558435579206764
-0.558435579206764 -0.558435579206764
-0.558435579206764 -0.635385594645107
-0.635385594645107 -0.635385594645107
-0.635385594645107 -0.556492562864909
-0.556492562864909 -0.556492562864909
-0.556492562864909 -0.623970391589078
-0.623970391589078 -0.623970391589078
-0.623970391589078 -0.571260388880268
-0.571260388880268 -0.571260388880268
-0.571260388880268 -0.601676528037732
};
